On Evaluating the Renaissance Benchmarking Suite: Variety, Performance, and Complexity

The recently proposed Renaissance suite is composed of modern, real-world, concurrent, and object-oriented workloads that exercise various concurrency primitives of the JVM. Renaissance was used to compare performance of two stateof-the-art, production-quality JIT compilers (HotSpot C2 and Graal), and to show that the performance differences are more significant than on existing suites such as DaCapo and SPECjvm2008. In this technical report, we give an overview of the experimental setup that we used to assess the variety and complexity of the Renaissance suite, as well as its amenability to new compiler optimizations. We then present the obtained measurements in detail.

==> experiments/atomic-operation-coalescing.tex <==
% !TEX root = ../main.tex
\small
\quad
\begin{tikzpicture}[scale=0.78]
  \begin{axis}[
  height=3.4cm,
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$ms$,
  xlabel=,
  grid=both,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=-8,
    yshift=-12,
    anchor=south,
  },
  every axis x label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=12,
    yshift=-10,
    anchor=north,
    rotate=0,
  },
  scaled y ticks=false,
  yticklabel style={
    /pgf/number format/fixed,
  },
  xticklabel style={
    rotate=0,
  },
  ytick={500, 1000, 1500, 2000, 2500},
  ybar=0.1pt,
  bar width=6pt,
  x=0.63cm,
  ymin=0,
  ymax=3600,
  x,
  axis on top,
  xtick=data,
  xtick=\empty,
  symbolic x coords={
    100k
  },
  % restrict y to domain*=0:75,
  visualization depends on=rawy\as\rawy,
  after end axis/.code={
    \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=1,
    at={(-0.05, 1.50)},
    anchor=north west
  },
  draw opacity=0.4,
  major grid style={
    draw opacity=0.3,
  },
]
    
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(100k, 2250)
};
\addlegendentry{without}
\node[above] at ($(axis cs:100k, 2250)$) [xshift=-0.45*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};

\addplot[
  fill={rgb:red,1;green,3;blue,1},
    postaction={
      pattern color=white,
      pattern=north east lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(100k, 1820)
};
\addlegendentry{with}
\node[above] at ($(axis cs:100k, 1820)$) [xshift=0.55*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$0.8\times$}}};
\end{axis}
\end{tikzpicture}

==> experiments/loop-wide-lock-coarsening.tex <==
% !TEX root = ../main.tex
\small
\quad
\begin{tikzpicture}[scale=0.78]
  \begin{axis}[
  height=3.8cm,
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$ms$,
  xlabel=,
  grid=both,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=-8,
    yshift=-12,
    anchor=south,
  },
  every axis x label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=12,
    yshift=-10,
    anchor=north,
    rotate=0,
  },
  scaled y ticks=false,
  yticklabel style={
    /pgf/number format/fixed,
  },
  xticklabel style={
    rotate=0,
  },
  ytick={300, 600, 900, 1200},
  ybar=0.1pt,
  bar width=6pt,
  x=0.63cm,
  ymin=0,
  ymax=1700,
  x,
  axis on top,
  xtick=data,
  xtick=\empty,
  symbolic x coords={
    100k
  },
  % restrict y to domain*=0:75,
  visualization depends on=rawy\as\rawy,
  after end axis/.code={
    \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=1,
    at={(-0.05, 1.40)},
    anchor=north west
  },
  draw opacity=0.4,
  major grid style={
    draw opacity=0.3,
  },
]
    
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(100k, 1160)
};
\addlegendentry{without}
\node[above] at ($(axis cs:100k, 1160)$) [xshift=-0.45*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};

\addplot[
  fill={rgb:red,1;green,3;blue,1},
    postaction={
      pattern color=white,
      pattern=north east lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(100k, 680)
};
\addlegendentry{with}
\node[above] at ($(axis cs:100k, 680)$) [xshift=0.55*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$0.6\times$}}};
\end{axis}
\end{tikzpicture}

==> experiments/virt-cas.tex <==
% !TEX root = ../main.tex
\small
\quad
\begin{tikzpicture}[scale=0.78]
  \begin{axis}[
  height=3.8cm,
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$ms$,
  xlabel=,
  grid=both,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=-8,
    yshift=-12,
    anchor=south,
  },
  every axis x label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=12,
    yshift=-10,
    anchor=north,
    rotate=0,
  },
  scaled y ticks=false,
  yticklabel style={
    /pgf/number format/fixed,
  },
  xticklabel style={
    rotate=0,
  },
  ytick={600, 1200, 1800, 2400, 3000},
  ybar=0.1pt,
  bar width=6pt,
  x=0.63cm,
  ymin=0,
  ymax=3800,
  x,
  axis on top,
  xtick=data,
  xtick=\empty,
  symbolic x coords={
    100k
  },
  % restrict y to domain*=0:75,
  visualization depends on=rawy\as\rawy,
  after end axis/.code={
    \draw[line width=3pt, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
  },
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=1,
    at={(-0.05, 1.40)},
    anchor=north west
  },
  draw opacity=0.4,
  major grid style={
    draw opacity=0.3,
  },
]
    
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(100k, 2470)
};
\addlegendentry{without}
\node[above] at ($(axis cs:100k, 2470)$) [xshift=-0.45*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};

\addplot[
  fill={rgb:red,1;green,3;blue,1},
    postaction={
      pattern color=white,
      pattern=north east lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(100k, 1880)
};
\addlegendentry{with}
\node[above] at ($(axis cs:100k, 1880)$) [xshift=0.55*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$0.76\times$}}};
\end{axis}
\end{tikzpicture}

==> sections/abstract.tex <==
% !TEX root = ../main.tex


Established benchmark suites for the Java Virtual Machine (JVM),
such as \mbox{DaCapo}, \mbox{ScalaBench}, and \mbox{SPECjvm2008},
lack workloads that take advantage of the parallel programming abstractions
and concurrency primitives offered by the JVM and the Java Class Library.
However, such workloads are fundamental for understanding the way in which
modern applications and data-processing frameworks use the JVM's concurrency features,
and for validating new just-in-time (JIT) compiler optimizations
that enable more efficient execution of such workloads.
We present \emph{Renaissance}, a new benchmark suite composed of
modern, real-world, concurrent, and object-oriented workloads
that exercise various concurrency primitives of the JVM.
We show that the use of concurrency primitives in these workloads
reveals optimization opportunities that were not visible with the existing workloads.
% This makes Renaissance better suited for evaluating JVM performance
% when executing modern concurrent applications,
% and also for better understanding of the workload exerted on the JVM by such applications.
% \gd{maybe remove this sentence?}
We use Renaissance to compare performance of two state-of-the-art,
production-quality JIT compilers (HotSpot C2 and Graal),
and show that the performance differences are more significant
than on existing suites such as DaCapo and SPECjvm2008.
We also use Renaissance to expose four new compiler optimizations,
and we analyze the behavior of several existing ones.
% Evaluating these optimizations using four benchmark suites
% shows speedups of up to $1.Y\times$ \gd{missing number} for the Renaissance workloads,
% while the existing workloads from the other suites, which do not take advantage
% of the modern concurrency primitives, show no significant effects.
% \lb{If that's how we would put it.}
Evaluating these optimizations using four benchmark suites shows
a more prominent impact on the Renaissance workloads than on those of other suites.

% \wb{
% Maybe add a final sentence about who are the beneficiaries of Renaissance
% (or in the conclusion).
% }
% \ap{Added in the conclusion.}


==> sections/benchmarks.tex <==
% !TEX root = ../main.tex

Our work has several motivating factors.
First, we realized that the state-of-the-art JIT compilers,
such as C2 and Graal, have very comparable performance, e.g., on the \mbox{DaCapo} suite,
and that it has become extremely difficult to demonstrate significant performance gains on the existing workloads when exploring new compiler optimizations.
Second, we determined that many modern programming abstractions, such as Java Lambdas~\cite{jsr335}, Streams~\cite{jep107}, or Futures~\cite{jep266},
were not represented in the existing benchmark suites.
Moreover, we found that the optimizations in existing JIT compilers
rarely focused on concurrency-related primitives.

\subsection{Selection Methodology}
\label{sec:selection-methodology}

To identify a core set of benchmarks which would reflect the use of modern
concurrency-related abstractions and programming paradigms, we manually
collected a large number of candidate workloads using popular Java and
Scala frameworks.
In addition to manual filtering, we also developed a tool, inspired by the
AutoBench toolchain~\cite{conf/wcre/ZhengRSLSJBCQB16}, to scan the online
corpus of open-source projects on GitHub\footnote{We included
GitHub projects with updates in the last 3 years (2015--2017) and higher number of 
recent commits, pull requests, and number of stars.} for candidate workloads.
When selecting benchmarks for the Renaissance suite, our main goals were as follows.

% \ap{Previously, the goals we had listed were:
% 1. ensure that the benchmarks represent realistic Java and Scala workloads.
% 2. Ensure that the benchmarks heavily exercise modern concurrent and parallel programming patterns.
% 3. Finally, the benchmarks should be relatively easy to use.
% Walter left several comments listed below, based on which I redid the section.
% }

% \wb{Why is [3.] an issue, isn't it the task of the harness to run the benchmarks? So this point would only simplify our harness, which doesn't seem to be a big deal.}

% \wb{What about diversity?}

% \wb{What about determinism of the benchmarks? In concurrent workloads, there is some inevitable non-determinism due to non-deterministic thread scheduling. However, we really want to minimize other sources of non-determinism as much as possible, isn't it?}

% \wb{In addition to avoiding workloads with (certain kinds of) non-determinism, we should also exclude workloads with other undesirable properties. For example, as we target concurrent workloads, it'd be useful to run an exact data-race detector (not prone to false positives) and to exclude applications with data races; similarly, running a dynamic analysis for generalized deadlock detection would be useful. This could be a discussion point regarding a toolchain that helps us filter out problematic workloads early in the benchmark-suite creation process.}

% \wb{What about open-source availability? This would allow researchers to apply various tools at the source-code level, and also to evaluating a profiler, showing that the profiles are actionable by optimizing the identified code segments. Moreover, it is important to provide metadata for each benchmark, detailing the complete build chain used to geenrate the bytecode (particularly the version of the Java or Scala compiler); we probably should also provide a snapshot of the whole toolchain to build the benchmarks.}

% \wb{Avoiding benchmarks that use timers may be also important to enable heavyweight instrumentations that can cause high runtime overheads (and so trigger timeouts). I think DaCapo daytrader is an example of such a problem. Generally, I think we should mention that we try to avoid flaws that were found with existing benchmark suites over the time, including timeout issues, non-availability of sources, memory leaks in benchmarks (imparing later benchmark iterations), etc.}

\paratitle{Modern Concurrency}
Benchmarks in the suite should rely on different styles of
concurrent and parallel programming. These include data-parallelism,
task-parallelism, streaming and pipelined parallelism,
message-based concurrency, software transactional memory,
lock-based and lock-free concurrent data structures and in-memory databases,
as well as asynchronous programming and network communication.

\paratitle{Realistic Workloads}
Benchmarks should reflect real-world applications.
To this end, we focused on workloads using popular Java and
Scala frameworks, such as Java Stream API~\cite{jep107},
Apache Spark~\cite{Zaharia:2010:SCC:1863103.1863113},
the Java Reac\-tive Ex\-ten\-sions~\cite{rx,rxjava},
the Java Fork/Join frame\-work~\cite{Lea:2000:JFF:337449.337465},
ScalaSTM~\cite{scala-stm-expert-group},
and Twitter Finagle~\cite{github-finagle}.
We reused existing workloads where possible, and we adopted several
standalone benchmarks that target specific paradigms,
such as STMBench7~\cite{Guerraoui:2007:SBS:1272996.1273029},
J. Paumard's Scrabble benchmark~\cite{scrabble-benchmark},
and the CloudSuite MovieLens benchmark for Apache Spark~\cite{Ferdman:2012:CCS:2248487.2150982}.
Overall, we collected roughly 100~benchmarks
since starting the effort in 2016.

\paratitle{Workload Diversity}
Benchmarks should be sufficiently diverse so that they exercise different concurrency-related features of the JVM, such as atomic instructions, Java §syn\-chro\-nized§ blocks, thread-park operations, or guarded blocks (i.e., the
§wait§-§notify§ pattern).
At the same time, the benchmarks should be object-oriented to exercise
the parts of the JVM responsible for efficient execution of code patterns
commonly associated with abstraction in object-oriented programs, i.e.,
frequent object allocation and virtual dispatch.
To this end, we analyzed candidate projects by running their testing code
and recording various concurrency-related metrics (\forcameraready{details in Section~\ref{sec:metric-comparison}})
to ensure adequate coverage of the metric space. This served as the basis
for the diversity analysis presented in Section~\ref{sec:pca}.

\paratitle{Deterministic Execution}
Benchmarks should behave in a deterministic fashion, even though it is not
possible to achieve full determinism in a suite focusing on concurrent
benchmarks due to non-determinism inherent to thread scheduling.
However, apart from that, the control flow of a benchmark should not include
non-deterministic choices on data produced, e.g., by a random generator
seeded by the current time instead of a constant.

\paratitle{Open-Source Availability}
Benchmarks should be open-source, and rely only on open-source frameworks,
whenever possible. This goal is important for several reasons.
First of all, it enables inspection of the workloads by the community and
allows multiple parties to collaborate on improving and maintaining the
suite so that it can evolve along with the target platform ecosystem.
Moreover, it enables source-code level analysis of the benchmarks, and
allows evaluating the actionability of profiler results.
And last, but not least, open-source software is less likely to
cause licensing issues.

\paratitle{Avoiding Known Pitfalls}
The benchmarks should avoid pitfalls that were identified in other benchmark suites
over time and which hinder adoption in a broader community. The lack of benchmark
source code is one such pitfall. Another pitfall is the use of timeouts, which
make it difficult to analyze the benchmark execution using dynamic analysis tools
that require heavy-weight instrumentation, because the timeouts keep triggering due
to high overhead. Yet another pitfall is benchmark correctness, avoiding benchmarks
with resource leaks and, especially in the case of concurrent benchmarks, data
races and deadlocks.

%\ar{I think the focus should be reviewed:
%1) make sure that it is not in contrast with actual metrics profiled,
%2) should we remove references to fast/slow/biased locks?
%They still appear in the table, I am not sure they were covered in text.
%3) Do you mean synchronized instead of synchronize?} }% summary 
%ar{Please add missing default number of repetitions to this table} \ar{Sort alphabetically?}
\subsection{Renaissance Benchmarks and Harness}
\label{sec:benchmark-descriptions}

\input{content/benchmarks}

The set of benchmarks that we ultimately decided to include in the Renaissance suite is shown
in Table~\ref{tab:benchmarks}, along with short descriptions.
In total, 14 out of 21 benchmarks were adapted from existing standalone benchmarks
(¡akka-uct¡, ¡als¡, ¡chi-square¡, ¡dec-tree¡,
¡fj-kmeans¡, ¡log-regression¡, ¡movie-lens¡, ¡naive-bays¡,
¡philosophers¡, ¡reactors-savina¡, ¡rx-scrabble¡, ¡scrabble¡,
¡stm-bench7¡ and ¡streams-mnemonics¡),
and the rest were gathered from production usages of different companies,
and usages in existing applications.

All benchmarks run within a single JVM process, and only rely on the JDK
as an external dependency.
Some of the benchmarks use network communication, and they are encoded as
multiple threads that exercise the network stack within a single process
(using the loopback interface).
We realize that this does not reflect realistic network conditions, but
it does exercise code responsible for spanning multiple address spaces,
which is common for data-parallel computational frameworks.
The default execution time of each benchmark is tuned to take several seconds.

We provide a harness that allows to run the benchmarks and collect
the results, and also allows to easily add new benchmarks.
The harness also provides an interface for custom measurement plugins,
which can latch onto benchmark execution events to perform additional
operations. For example, most of the metrics in Section~\ref{sec:metric-comparison}
were collected using custom plugins.
In addition, the harness allows running the benchmarks with JMH~\cite{jmh}
(a standard microbenchmarking tool for the JVM) as a frontend to avoid
common measurement pitfalls associated with benchmarking.

% TODO N benchmarks focus on data-parallel workloads,
% using either Java 8 Streams~\cite{jep107}
% or Apache Spark~\cite{Zaharia:2010:SCC:1863103.1863113}.
% The task-parallel workloads, ¡fj-kmeans¡ and ¡future-genetic¡,
% rely on the Fork/Join framework~\cite{Lea:2000:JFF:337449.337465}
% and Java futures~\cite{jep266}.
% The message-based concurrency benchmarks rely Akka~\cite{akka},
% Reactors framework for Scala~\cite{Prokopec:2015:ICE:2814228.2814245}
% and the Finagle HTTP framework~\cite{github-finagle},
% while the STM workloads use ScalaSTM~\cite{Bronson10ccstm:a,scala-stm-expert-group}.


==> sections/comparison.tex <==
% !TEX root = ../main.tex

%\ar{These are the metrics that drove the benchmark selection process.
%Shall we give them some more important name? `Representative metric'? `
%Key metric'? Naming the section just `Metric' looks a bit reductive.}
%\ap{Some ideas: "distinguishing", "distinctive", "characterizing". I like "key metrics" too.}
%\ap{
%One small request, btw: would it be a problem to wrap
%the text parts of the Latex source at 96 characters?
%It would make it easier to read on a laptop without having to scroll left-and-right.
%I think its fine if tables, long URLs and similar aren't wrapped, but main text would be nice.
%}

%\ar{This and the following section talk about ``concurrency metrics'',
%not ``parallelism metrics''. Change text at a later time if needed}

To meet the goals outlined in Section~\ref{sec:selection-methodology},
we define a set of metrics to characterize the usage of concurrency primitives,
basic primitives of object-oriented programming,
and modern programming primitives introduced in JDK 7 or later.
Notably, our goal is not to define an exhaustive set of metrics to cover all of these features.
Instead, we aim at profiling metrics that
1) can reasonably characterize the use of these features,
2) can be collected with simple instrumentation, and
3) can be easily understood.

In this section, we present the metrics used in benchmark selection,
and the details of how we collect them.
Subsequent sections compare these metrics across different benchmarks
and relate them with compiler optimizations.

%\wb{Dynamic compiler? JIT compiler? Or maybe better, mention in the beginning that in this paper,
% compiler stands for JIT compiler (though there is a problem if we also need the terms Java compiler, Scala compiler...}

%\ar{Expand the last sentence at a later time if needed.}

%\ap{
%Small note: we should use consistent benchmark naming throughout all sections
%(I suggest using the names from Table 1).
%}

%~(\autoref{subsec:metric:desc}); then, we show that Renaissance is more more parallel- and concurrent- oriented than other existing benchmark suites, while still executing non-trivial workloads~(\autoref{subsec:metric:pca}).


\subsection{Description of the Metrics}
\label{subsec:metric:desc}

%\begin{table}
%  \caption{Metrics considered in the benchmark selection process. }
%  \label{tab:metrics}
%  % \small
%  \footnotesize
%\begingroup
%\setlength{\tabcolsep}{10pt} % Default value: 6pt
%\renewcommand{\arraystretch}{1.2} % Default value: 1
%  \begin{tabular}{
%    l@{\hskip0.2cm} L{5.9cm} %c
%  }
%    \toprule
%    Name & Description \\%& Norm.\\
%%    \midrule
%%    \multicolumn{2}{c}{Parallelism}\\
%%    \midrule
%synch	&	§synchronized§ methods and blocks executed.\\ %& \pmark\\
%%n-locks	&	Yes	Total number of calls to lock(), lockInterruptibly(), tryLock() (defined in class java.util.concurrent.locks.Lock)
%wait	&	Invocations to §Object.wait()§.\\% & \pmark\\
%notify	&	Invocations to §Object.notify()§ and §Object.notifyAll()§.\\ %& \pmark\\
%atomic	&	Atomic operations executed (compare-and-swap, get-and-set, get-and-add).\\ %& \pmark\\
%park	& Park operations.\\% & \pmark\\
%biased-lock & Biased, rebiased, and anonymously biased locks acquired.
%\ar{Gilles, Shall we mention all this kinds of biased locks?}
%\ap{
%I think it depends on which PCA we choose.
%Maybe you could additionally try a PCA with only biased and fast locks,
%since the slow path locks are anyway not very represented in absolute terms
%(plus, in some of your recent PCA versions, they seem to have obtained a high score).
%}\\ % & \pmark\\
%fast-lock & Fast path locks acquired.\\ %& \pmark\\
%slow-lock & Slow path locks acquired.\\ %& \pmark\\
%avg-cpu	&	Average CPU utilization (user and kernel).\\% & \xmark\\
%cache-miss	 &	Cache misses, including L1 cache (instruction and data), last-layer cache (LLC)
%and translation lookaside buffer (TLB; instruction and data).\\% & \pmark\\
%%\midrule
%%    \multicolumn{2}{c}{Other}\\
%%    \midrule
%object	& Objects allocated.\\ %& \pmark\\
%array 	& Arrays allocated.\\ %& \pmark\\
%method	& Methods invoked.\\ %& \pmark\\ 
%invokedynamic&  §invokedynamic§ bytecodes executed.\\ %& \pmark\\
%\bottomrule
%\end{tabular}
%\endgroup
%\end{table}



%%%%%%% THE TABLE BELOW INTEGRATES PCA RANKING.
%%%%%%% UNCOMMENT IT IF NEEDED


%\begin{table}
%  \caption{Metrics considered in the benchmark selection process and their rank in the four principal components (PC).}
%  \label{tab:metrics}
%  \footnotesize
%\begingroup
%  \begin{tabular}{
%    l@{\hskip0.2cm} p{4cm} l@{\hskip-0.05cm} r r r r%c
%  }
%    \toprule
%    \multirow{2}{*}{Name} & \multirow{2}{*}{Description}     & \multicolumn{5}{c}{PC$i$ Rank}\\
%    \cline{3-7}
%& &$i$& {\tt1} & {\tt2} &  {\tt3} & {\tt4}\\
%    \midrule
%\metric{synch}	&	§synchronized§ methods and blocks executed && {\tt -6} &	{\tt-10}	&{\tt-5}	&{\tt+10}\\
%\hdashline[0.5pt/1pt]
%\metric{wait}	&	Invocations of §Object.wait()§ && {\tt-11}&	{\tt-11}&	{\tt+3}	&{\tt-8}\\
%\hdashline[0.5pt/1pt]
%\metric{notify}	&	Invocations of §Object.notify()§ and §Object.notifyAll()§ && {\tt-7}	&{\tt+4}	&{\tt+2}	&{\tt+3}\\
%\hdashline[0.5pt/1pt]
%\metric{atomic}	&	Atomic operations executed (compare-and-swap, get-and-set, get-and-add) && {\tt-8}	&{\tt+1}&	{\tt-11}&	{\tt+7}\\
%\hdashline[0.5pt/1pt]
%\metric{park}	& Park operations && {\tt-10}&{\tt+2}&	{\tt-6}&	{\tt+11}\\
%\hdashline[0.5pt/1pt]
%\metric{cpu}	&	Average CPU utilization (user and kernel) && {\tt-2}	&{\tt-6}	&{\tt-4}	&{\tt+6}\\
%\hdashline[0.5pt/1pt]
%\metric{cachemiss}	 &	Cache misses, includinge L1 cache (instruction and data), last-layer cache (LLC),
%and translation lookaside buffer (TLB; instruction and data) && {\tt-9}	& {\tt-7}	& {\tt+1}	& {\tt+5}\\
%\hdashline[0.5pt/1pt]
%\metric{object}	& Objects allocated & &{\tt+1}	&{\tt+8}	&{\tt-10}&	{\tt+9}\\
%\hdashline[0.5pt/1pt]
%\metric{array} 	& Arrays allocated &&{\tt+4}	&{\tt-9}&	{\tt-8}&	{\tt+2}\\
%\hdashline[0.5pt/1pt]
%\metric{method}	& Methods invoked &&{\tt+3}	&{\tt+3}	&{\tt+9}	&{\tt-4}\\
%\hdashline[0.5pt/1pt]
%\metric{idynamic}& §invokedynamic§ bytecodes executed &&{\tt+5}	&{\tt-5}	&{\tt-7}	&{\tt+1}\\
%\bottomrule
%\end{tabular}
%\endgroup
%\end{table}

%%%%%%%
%%%%%%%

\input{content/metrics.tex}

Table~\ref{tab:metrics} presents the metrics used during benchmark selection.
The initial several metrics in the list
reflect the usage of some basic concurrency primitives on the JVM~\cite{jsr133}:
(1)~§synchronized§ blocks and methods (i.e. critical sections),
(2)~§wait§/§notify§ calls (i.e. guarded blocks),
(3)~atomic memory-access operations (e.g., compare-and-swap),
(4)~thread parking and unparking.
Since most high-level concurrency abstractions are implemented from these basic primitives,
their usage rates estimate the use of concurrency abstractions during execution.
We therefore collect the dynamic invocation counts of these primitives\footnote{
  We omitted unparks, since they correlated with \metric{park}s in all benchmarks.
}.

%\wb{The previous table doesn't mention unpark.}
%\wb{Are volatiles variables covered? I'd sggest to mention them before the atomic variables.}
%\wb{Most or all? If not all, which primitives are we missing?}
%\ar{Alex, do you think that the included primitives can cover all high-level concurrency abstractions?}
%\ap{
%I think that any usage of *most* high-level concurrency abstraction
%should increment at least one of the counters that we selected.
%There are some exceptions that I can think of at the moment:
%(1) a native call or some JDK call that ends up calling a kernel synchronization primitive,
%(2) Java NIO and networking,
%(3) fences and some other Unsafe API usages (note Unsafe was extended a lot, but after JDK8).
%}
 %\wb{``Level of concurrency'' is fuzzy, either define this term properly, or better avoid it altogether.
 % Some people may consider the number of active threads to be the level of concurrency, for example.}
 %\ar{If needed, write in a footnote which kinds of primitive we don't track.}
% \ap{
%I think that any usage of *most* high-level concurrency abstraction
%should increment at least one of the counters that we selected.
%There are some exceptions that I can think of at the moment:
%(1) a native call or some JDK call that ends up calling a kernel synchronization primitive,
%(2) Java NIO and networking,
%(3) fences and some other Unsafe API usages (note Unsafe was extended a lot, but after JDK8).
%}
%
  %synchronization and inter-thread communication.
% \wb{How do you define inter-thread communication in this paper?
% Is it the access to shared variables? In this case, what about code that piggybacks
% on synchronization? It should be also seen as inter-thread communication, but wouldn't be included in the above metrics.}
%A particularly high usage rate suggests that the primitive
%is used in a \emph{hot} part of the application,
%where optimizing it can potentially noticeably improve performance.
% \ar{I commented the above sentence, because I think it fits better
% in Section 5 (i.e., in section 5 you can motivate further the inclusion
%of this metric.
%
%\wb{dynamic instead of total?}

%\wb{When you worked on tgp, wasn't one of the early findings that
% cache misses were not a good metric to capture contention?}
%\ar{Find a proper justification for cache-misses}
%\wb{Also a single-threaded workload may suffer from a very high number of cache misses, if locality is bad (e.g., random accesses in a huge data structure).}
%\ar{The list of metric in the table should be refined. Are we sure we really need them all?}

%\ap{
%Maybe you can say that synchronization primitives and VM facilities
%must be optimized differently depending on the contention level. For example:
%1. without the interaction of multiple threads, all locks become biased on the JVM.
%2. without multiple threads, no contention effects due to writing to the same location (MESI).
%3. similarly, false-sharing (due to memory layout, or even card-marking --
%   see "dave dice card marking") cannot be observed.
%4. without higher CPU utilization, the GC has more CPUs to work with.
%5. a single thread is unlikely to exercise the wait aspect of the wait-notify monitor.
%}


%
%- CPU utilization
%
%- biased/fast-path/slow-path locking
%\ar{}
%
%- cache-miss rates
%\ar{Could it track the amount of contention?}
%\ap{
%L1 cache misses might in theory, but I'm not sure if
%a cache-line state change in the MESI protocol shows up in the cache miss count.
%}
%
%Finally, ...

%\ar{
%These are not really metrics related to concurrency... Shall we discuss them somewhere else?
%}
%\ap{I would instead rephrase the title of the section.}

Next, we define a metric for the average CPU utilization,
and a metric for the number of cache misses during execution.
Both these metrics are indirectly related to concurrency -- for example,
unless several CPUs or cores are utilized by the benchmark,
it is unlikely that the benchmark will exhibit
interesting synchronization behavior.
Similarly, a high cache-miss rate may indicate contention between threads.

Then, we track the object-allocation rate, the array-alloca\-tion rate,
and the dynamic-dispatch rate
(i.e., the execution counts of the
{\tt invokedynamic}, {\tt invokeinterface}, or {\tt invokevirtual} bytecodes).
These metrics estimate the usage of the basic primitives in object-oriented programming,
and usually correlate with the complexity of the code\footnote{
  Some data-parallel and streaming frameworks allocate intermediate arrays.
}.
%\wb{Explicitly list the bytecodes considered to indicate that
%invokedynamic is excluded here.},
%\wb{The last statement is simply not true and opens us up to easy attacks. In particular, the invocation metric is convoluting dynamic and static binding.}
%, which in turn are an indication of
% realistic object-oriented JVM applications.
%\wb{That's a very strong claim (real-world OO applications can be identified only by looking at three counters. If this claim remains, a reference is needed.}
%\ar{However, array allocations are not a measure of abstractions offered by OOP...}
%\ap{
%That's not entirely true -- for example, in Jenetics and in Scala,
%the "map" method allocated intermediate arrays, which could be optimized away
%if we had a better loop fusion in Graal.
%}
%\ap{(We discussed this a lot on the meeting yesterday)}
% We also track the number of arrays allocated at runtime, as a measure of
%\ar{? It is hard to claim that arrays are a measure of abstractions.
%The real reason is that array probably have an impact on compiler optim. }

%We also track
%We collect this metric because common operations used in big-data processing
%(such as maps) allocates arrays during intermediate

Finally, we track the execution rate of the §invokedynamic§ bytecode
(introduced in JDK 7~\cite{jsr292}),
which supports dynamic languages on the JVM~\cite{6493308},
and is also used to implement Lambdas~\cite{jsr335}.
Java Lambdas are used in various data-processing libraries --
for example, Java Streams~\cite{jep107} or Reactive Extensions~\cite{rx}
expose operations such as §map§ and §reduce§
that typically take Lambda values as arguments.
Therefore, counting the §invokedynamic§ occurrences allows estimating
the usage rate of high-level operations.

% Moreover, §invokedynamic§ is used in programming patterns introduced
% in Java~7 or after, such as
% method handles (i.e., typed executable
% references to a method, constructor or field~\cite{methodhandle}) or
% Java Streams~(i.e., classes supporting functional-style operations~\cite{streams})
% not found in
% other benchmark suites. Finally, since, in some frameworks,
% some intermediate operations such as §map§ allocate arrays,
% we track the number of array allocations as well,
% as a measure to distinguish workloads making use of such operations.

%\ar{Is there any other usage of invokedynamic?}
%\ap{There are many usages, so it's a necessary condition for Streams, Rx, etc.,
%but does not exclude others (e.g. that some benchmark is calling JRuby,
%although that particular example is unlikely).}

%... TODO ... why did we choose object allocations,
%
%... TODO ... invokedynamic, new bytecode instruction, appears a lot in ...

%- context switches -- we chose not to include them \ar{Not exclusively related to concurrency, maybe we can avoid mentioning?}
%
%- volatile accesses -- we chose not to include them

%\ap{We should include some justification for context switches and volatile accesses.}


\subsection{Normalization}

When collecting the metrics from Table \ref{tab:metrics},
absolute values are not very indicative,
since a high value may reflect a long execution rather than
a frequent usage of a given primitive, which is our focus.
To this end, we use rates rather than absolute values,
and we normalize each metric (except \metric{cpu})
by the total amount of \emph{references cycles} executed by the benchmark,
\forcameraready{
defined as machine cycles that are measured at a constant nominal frequency,
even if the real CPU frequency scales up or down~\cite{rc-def}.
}


We use reference cycles as a measure of the amount of computations executed by an application.
%A reference cycle always elapses at the nominal CPU frequency,
%even if the frequency changes
% by the operating system (OS) \wb{Is the OS setting the frequency?}
%during program execution.
Using reference cycles allows comparing the metrics between different benchmarks,
even if they are executed under different or fluctuating CPU frequencies.
Moreover, reference cycles represent runtime conditions more accurately,
since they account for instruction complexity
(as complex instructions take more cycles)
and for latencies due to e.g.~cache misses.

%\wb{Is the OS setting the frequency?}
%\ap{
%To my understanding, the frequency is set by at least 2 entities.
%First the Intel P-State driver, which can be replaced with a different driver,
%does this by following the user-modifiable governor policy, as best as possible
%(https://www.kernel.org/doc/Documentation/cpu-freq/intel-pstate.txt).
%I sometimes disable Intel P-State to measure performance
%(there is a boot option on Linux).
%Second, the CPU itself has some built-in facilities for reducing the frequency.
%If the temperature exceeds a certain level, then the frequency is reduced
%regardless of the driver does.
%}

%We choose reference cycles among other possible normalization bases
%(such as wall time or number of bytecode/machine instructions executed)
%because cycles


\subsection{Metric Collection}\label{subsec:metrics:collection}
%\ar{I think it would be strange to not explain how we collect the metrics,
%although I am not sure we should really mention everything.
%We can use it to motivate the exclusion of fast/slow/biased lock from
%PCA. If there is no space, we can move it to appendix}
%\ap{Agreed, we should describe it here.}

To collect the metrics, we rely on different tools.
To profile the usage of concurrency primitives
(\metric{synch}, \metric{wait}, \metric{notify}, \metric{atomic}, \metric{park}),
allocations (\metric{object}, \metric{array}),
invocations (\metric{method}), and §invokedynamic§ executions (\metric{idynamic}),
we developed a profiler based on bytecode instrumentation,
built on top of the open-source dynamic
program-analysis framework \prog{DiSL}\footnote{
  \url{https://disl.ow2.org/}
}~\cite{Marek:2012:DDL:2162049.2162077}.
The profiler exploits the full bytecode coverage offered by \prog{DiSL}
(i.e., it can instrument every method which has a bytecode representation),
so the metrics can be collected in every loaded class,
including the classes of the Java class library,
as well as the classes that are dynamically generated or fetched from a remote location.
The profiler uses a deployment setting of \prog{DiSL} called
\prog{Shadow~VM}~\cite{Marek:2013:ShadowVM} to enforce isolation
between analysis and application code, preventing certain well-known problems
that may be introduced by less isolated approaches~\cite{Kell:2012:JVM}.
We profile \metric{atomic} and \metric{park} by intercepting the respective method
calls in §sun.misc.Unsafe§.
CPU utilization is sampled periodically every $\sim$150ms using \prog{top}~\cite{top}.
Finally, we use \prog{perf}~\cite{perf} to collect cache misses
and reference cycles (used for normalization).
While instrumentation may influence thread interleaving and bias the collection,
we made sure to keep the perturbations low
with minimal instrumentation that avoids heap allocations,
and by keeping the profiling data structures in a separate process, on a separate NUMA node.
Additional details on the experimental setup
can be found in Section~\ref{sec:app:pca:settings} of the supplemental material.


%\wb{
% Talk about measurement perturbations.
% I assume you are collecting the metrics in several runs,
% as collecting low-level metrics for an instrumented application
% could create a severe bias in the results
%}


%\subsection{Experimental Setup}

%We collect concurrency-related metrics (\metric{synch}, \metric{wait},
%\metric{notify}, \metric{atomic}, \metric{park}), in the second run, we collect
%abstractions-oriented metric (\metric{object}, \metric{array}, \metric{method}) and
%§invokedynamic§ usages (\metric{idynamic}). In the final one, we collect OS- and
%hardware-layer metrics (\metric{cpu}, and \metric{cachemiss}). Our approach is





%\subsection{Comparison}
%
%... TODO ... compare suites on the most prominent metrics
%\ar{
%What is the sense of comparing the suite on the most prominent metrics,
%but still mentioning all others? What do we use them for? PCA only?
%Or, we should just mention that these metrics guided our selection of benchmarks,
%without providing more details?
%Then, maybe it is better to move the discussion in previous section.
%}
%\ap{
%1st question:
%Because we want to highlight the differences between the suites.
%2nd question:
%Even if other metrics show small differentiation,
%it still shows that Renaissance at least spans the metric space as well as the other suites.
%3rd question:
%I'm fine with including the comparison discussion in an earlier section.
%I think it's mostly up to you to decide how you want to organize Section 3.
%}
%




%\begin{figure*}[t]
%\centering
%\includegraphics[width=2\columnwidth]{figures/biasedLocks}
%\caption{
%Kinds of locks - Temporary figure
%\ar{Ratio of fast path locks is significant in renaissance. Is this good?}
%\ap{It might represent new optimization opportunities for the compiler.}
%\ap{One other comment -- relative counts aren't very useful, absolute counts tell more.}
%}
%\label{fig:biased_locks}
%\end{figure*}
%
%\begin{figure*}[t]
%\centering
%\includegraphics[width=2\columnwidth]{figures/cpu}
%\caption{
%CPU utilization - Temporary figure.
%\ar{Hard to justify results here. Maybe diversity? But, looks in contrast with other results}
%\ap{
%Renaissance generally has a higher CPU usage, except compared to SPECjvm2008.
%Question is: how does SPECjvm2008 achieve this CPU usage.
%Do they run the same workload in separate threads?
%Do those threads communicate or synchronize?
%}
%}
%\label{fig:cpu}
%\end{figure*}
%
%

%
%\begin{figure*}[t]
%\centering
%\includegraphics[width=2\columnwidth]{figures/wait}
%\caption{Total wait - Normalized by reference cycles elapsed. - Temporary figure
%\ar{Not so good...}
%}
%\label{fig:synch}
%\end{figure*}
%
%\begin{figure*}[t]
%\centering
%\includegraphics[width=2\columnwidth]{figures/notify}
%\caption{Total notify - Normalized by reference cycles elapsed. - Temporary figure }
%\label{fig:synch}
%\end{figure*}
%
%\begin{figure*}[t]
%\centering
%\includegraphics[width=2\columnwidth]{figures/park}
%\caption{Total park - Normalized by reference cycles elapsed. - Temporary figure
%\ar{Good...}
%\ap{Although hard to argue importance, e.g. where this metric relates to optimizations.}
%}
%\label{fig:synch}
%\end{figure*}
%
%\begin{figure*}[t]
%\centering
%\includegraphics[width=2\columnwidth]{figures/join}
%\caption{Total join - Normalized by reference cycles elapsed. - Temporary figure
%\ar{?}
%}
%\label{fig:synch}
%\end{figure*}
%
%\begin{figure*}[t]
%\centering
%\includegraphics[width=2\columnwidth]{figures/cachemisses}
%\caption{Total cache misses - Normalized by reference cycles elapsed. - Temporary figure
%\ar{?}
%}
%\label{fig:synch}
%\end{figure*}





%\ap{We should include invokedynamic usage here.}


==> sections/compiled-code-size.tex <==
% !TEX root = ../main.tex


\begin{figure}
\center
\includegraphics[scale=0.4]{../experiments/codesize/codesize.pdf}
\caption{Code Size Metrics}
\label{fig:code-size-metrics}
\end{figure}

This section presents several metrics about the size of the compiled programs.
Figure \ref{fig:code-size-metrics} shows the
code size and compiled-method count distribution
for the \mbox{DaCapo}, \mbox{ScalaBench}, SPEC\-jvm2008, 
and \mbox{Renaissance} suites.
Both the code size and the method count
refer to the hot code, compiled with the second-tier optimizing compiler,
and were measured using Oracle's Graal compiler \cite{graalvm-download}
by letting the benchmark run for 120 seconds.

The JVM uses the method's invocation count and its loop iteration counts
to decide if a method is hot (i.e. frequently executed).
Hot methods are compiled using the second-tier optimizing compiler,
so the total size and the method count of the hot code
indicate how much of the program was deemed important for the overall performance.

The geomean of the compiled code size (across all benchmarks)
is $\approx$6.87MB for Renaissance,
which is slightly lower than $\approx$7.98MB for DaCapo,
and $\approx$10.03MB for ScalaBench.
The geomean of the total number of hot methods
is $\approx$\numprint{1636} for Renaissance,
which is slightly higher than $\approx$\numprint{1599} for DaCapo,
and somewhat lower than $\approx$\numprint{1853} for Scalabench.

% Interestingly, we noticed that two of the ScalaBench benchmarks, ¡scalatest¡ and ¡specs¡,
% repetitively execute the classloading of the same bytecodes
% (concretely, the unit tests that are passed to those frameworks)
% in each iteration of the benchmark \cite{scalatest-classloading,specs-classloading}.
% Therefore, the compiled code size correlates with how long these benchmarks run,
% which is somewhat misleading.
% Without ¡specs¡ and ¡scalatest¡, the geomean of the code size is $\approx$8.36MB.
% The DaCapo's ¡jython¡ benchmark similarly generates and loads the same bytecodes,
% and excluding it brings DaCapo's geomean code size to $\approx$7.34MB.

While \mbox{DaCapo}, \mbox{ScalaBench} and \mbox{Renaissance} are roughly in the same range,
the \mbox{SPECjvm2008} has a geomean of $\approx$486 hot methods,
and a geomean code size of $\approx$1.17MB
(for readability, the names of individual SPECjvm2008 benchmarks
are not shown in Figure \ref{fig:code-size-metrics}).
This indicates that the \mbox{SPECjvm2008} workloads are considerably smaller.


==> sections/complexity.tex <==
% !TEX root = ../main.tex

In this section, we compare the software complexity and the compiled code size of Renaissance 
against the one of DaCapo, ScalaBench and SPECjvm2008.

\subsection{Software Complexity Metrics}
\label{sec:software-complexity-metrics}

%In this section, we compare Renaissance against DaCapo, ScalaBench and SPECjvm2008
Here, we compare Renaissance against the other benchmark suites
by computing the Chidamber and Kemerer (CK) metrics~\cite{chidamber1994metrics},
which were previously used to evaluate software complexity of benchmarks
from the \mbox{DaCapo} and \mbox{CD$_x$}~\cite{doi:10.1002/cpe.1677} suites.
We used the \emph{ckjm}~\cite{spinellis2005tool} tool to calculate the metrics.
To analyze only the classes used in each benchmark (and not all the classes in the classpath),
we also developed a JVMTI native agent~\cite{jvmti}
for the HotSpot JVM %~\cite{Paleczny:2001:JHT:1267847.1267848}
that receives class-loading events from the VM,
and forwards the loaded  classes to \emph{ckjm}, which then calculates the metrics.

We use the following CK metrics:
\\
\begin{enumerate*}[label=\arabic{*}.,itemsep=0mm,itemjoin=\hspace{-0.2mm}]
\item\label{enum:ck-wmc}\emph{Weighted methods per class} (\textbf{WMC}),
which is calculated as the number of declared methods per loaded class.
\\
\item\label{enum:ck-dit}\emph{Depth of the inheritance tree} (\textbf{DIT}),
defined as the depth of the inheritance tree along all loaded classes.
\\
\hspace{-1cm}
\item\label{enum:ck-noc}\emph{Number of children} (\textbf{NOC})
is computed as the number of immediate subclasses of a class.
\\
\hspace{-1cm}
\item\label{enum:ck-cbo}\emph{Coupling between object classes} (\textbf{CBO})
counts the number of classes coupled to a given class,
either by method calls, field accesses, inheritance, 
method signatures or exceptions.
\\
\hspace{-1cm}
\item\label{enum:ck-rfc}\emph{Response for a class} (\textbf{RFC})
counts the number of different methods that are
potentially (transitively) executed when a single method is invoked.
\\
\hspace{-1cm}
\item\label{enum:ck-lcom}\emph{Lack of cohesion} (\textbf{LCOM})
counts how many methods of a class are not related
by accessing the same field of that class.
\end{enumerate*}
\begin{table}[ht]
	\scriptsize
	\begin{tabular}{llrrrrrr}
	
		\hline
		
		\multicolumn{1}{l}{} &
		\multicolumn{1}{r}{\bf WMC} & 
		\multicolumn{1}{r}{\bf DIT} & 
		\multicolumn{1}{r}{\bf CBO} &
		\multicolumn{1}{r}{\bf NOC} & 
		\multicolumn{1}{r}{\bf RFC} & 
		\multicolumn{1}{r}{\bf LCOM}\\ 
	\hline
	
		
		\multicolumn{7}{c}{\bf Renaissance}\\ 	\hline
	
		
		\multicolumn{1}{l|}{min-sum}& 
		\multicolumn{1}{r}{\tt 21830}& 
		\multicolumn{1}{r}{\tt 3066}& 
		\multicolumn{1}{r}{\tt 21757}& 
		\multicolumn{1}{r}{\tt 1571}& 
		\multicolumn{1}{r}{\tt 41799}& 
		\multicolumn{1}{r}{\tt 455958} 
		\\
		\multicolumn{1}{l|}{max-sum}& 
		\multicolumn{1}{r}{\tt 206933}& 
		\multicolumn{1}{r}{\tt 23936}& 
		\multicolumn{1}{r}{\tt 184901}& 
		\multicolumn{1}{r}{\tt 14029}& 
		\multicolumn{1}{r}{\tt 369131}& 
		\multicolumn{1}{r}{\tt 7360650} 
		\\   
		
		
		\hdashline[0.5pt/1pt]
		
		\multicolumn{1}{l|}{geomean-sum}& 
		\multicolumn{1}{r}{\tt \textbf{55533}}& 
		\multicolumn{1}{r}{\tt \textbf{7842}}& 
		\multicolumn{1}{r}{\tt \textbf{55147}}& 
		\multicolumn{1}{r}{\tt \textbf{4212}}& 
		\multicolumn{1}{r}{\tt \textbf{105105}}& 
		\multicolumn{1}{r}{\tt 1358042} 
		\\ \hdashline[0.5pt/1pt]\hdashline[0.5pt/1pt]
		
		
		\multicolumn{1}{l|}{min-avg}& 
		\multicolumn{1}{r}{\tt 11.07}& 
		\multicolumn{1}{r}{\tt 1.79}& 
		\multicolumn{1}{r}{\tt 12.57}& 
		\multicolumn{1}{r}{\tt 0.97}& 
		\multicolumn{1}{r}{\tt 20.78}& 
		\multicolumn{1}{r}{\tt 141.02} 
		\\
		\multicolumn{1}{l|}{max-avg}& 
		\multicolumn{1}{r}{\tt 18.48}& 
		\multicolumn{1}{r}{\tt 2.29}& 
		\multicolumn{1}{r}{\tt 17.54}& 
		\multicolumn{1}{r}{\tt 1.16}& 
		\multicolumn{1}{r}{\tt 33.84}& 
		\multicolumn{1}{r}{\tt 706.54} 
		\\
		
		
		\hdashline[0.5pt/1pt]
		
		\multicolumn{1}{l|}{geomean-avg}& 
		\multicolumn{1}{r}{\tt 13.58}& 
		\multicolumn{1}{r}{\tt \textbf{1.92}}& 
		\multicolumn{1}{r}{\tt 13.49}& 
		\multicolumn{1}{r}{\tt 1.03}& 
		\multicolumn{1}{r}{\tt 25.71}& 
		\multicolumn{1}{r}{\tt 332.19} 
		\\
		
		
		
		
		\hline
		
		\multicolumn{7}{c}{\bf DaCapo~\cite{Blackburn:2006:DBJ:1167515.1167488}} \\ 	\hline
	
			

\multicolumn{1}{l|}{min-sum}& 
\multicolumn{1}{r}{\tt 12466}& 
\multicolumn{1}{r}{\tt 1687}& 
\multicolumn{1}{r}{\tt 10640}& 
\multicolumn{1}{r}{\tt 857}& 
\multicolumn{1}{r}{\tt 22378}& 
\multicolumn{1}{r}{\tt 161333} 
\\
\multicolumn{1}{l|}{max-sum}& 
\multicolumn{1}{r}{\tt 124191}& 
\multicolumn{1}{r}{\tt 5753}& 
\multicolumn{1}{r}{\tt 45597}& 
\multicolumn{1}{r}{\tt 6421}& 
\multicolumn{1}{r}{\tt 97757}& 
\multicolumn{1}{r}{\tt 616524} 
\\


\hdashline[0.5pt/1pt]
\multicolumn{1}{l|}{geomean-sum}& 
\multicolumn{1}{r}{\tt 32470}& 
\multicolumn{1}{r}{\tt 3377}& 
\multicolumn{1}{r}{\tt 23275}& 
\multicolumn{1}{r}{\tt 2160}& 
\multicolumn{1}{r}{\tt 48461}& 
\multicolumn{1}{r}{\tt 336192} 
\\
 
 \hdashline[0.5pt/1pt]\hdashline[0.5pt/1pt]


\multicolumn{1}{l|}{min-avg}& 
\multicolumn{1}{r}{\tt 11.74}& 
\multicolumn{1}{r}{\tt 1.24}& 
\multicolumn{1}{r}{\tt 11.90}& 
\multicolumn{1}{r}{\tt 0.97}& 
\multicolumn{1}{r}{\tt 22.07}& 
\multicolumn{1}{r}{\tt 130.36} 
\\
\multicolumn{1}{l|}{max-avg}& 
\multicolumn{1}{r}{\tt 42.43}& 
\multicolumn{1}{r}{\tt 2.13}& 
\multicolumn{1}{r}{\tt 14.45}& 
\multicolumn{1}{r}{\tt 2.19}& 
\multicolumn{1}{r}{\tt 32.27}& 
\multicolumn{1}{r}{\tt 310.86} 
\\		


\hdashline[0.5pt/1pt]

\multicolumn{1}{l|}{geomean-avg}& 
\multicolumn{1}{r}{\tt 17.97}& 
\multicolumn{1}{r}{\tt 1.87}& 
\multicolumn{1}{r}{\tt 12.88}& 
\multicolumn{1}{r}{\tt \textbf{1.20}}& 
\multicolumn{1}{r}{\tt 26.82}& 
\multicolumn{1}{r}{\tt 186.05} 
\\


		\hline
		
		\multicolumn{7}{c}{\bf ScalaBench~\cite{Sewe:2011:DCC:2048066.2048118}}\\ 	\hline
	
		

\multicolumn{1}{l|}{min-sum}& 
\multicolumn{1}{r}{\tt 24693}& 
\multicolumn{1}{r}{\tt 2657}& 
\multicolumn{1}{r}{\tt 19713}& 
\multicolumn{1}{r}{\tt 1481}& 
\multicolumn{1}{r}{\tt 45364}& 
\multicolumn{1}{r}{\tt 1080228} 
\\
\multicolumn{1}{l|}{max-sum}& 
\multicolumn{1}{r}{\tt 150895}& 
\multicolumn{1}{r}{\tt 7789}& 
\multicolumn{1}{r}{\tt 66036}& 
\multicolumn{1}{r}{\tt 7890}& 
\multicolumn{1}{r}{\tt 124240}& 
\multicolumn{1}{r}{\tt 2298594} 
\\

\hdashline[0.5pt/1pt]
\multicolumn{1}{l|}{geomean-sum}& 
\multicolumn{1}{r}{\tt 44505}& 
\multicolumn{1}{r}{\tt 4291}& 
\multicolumn{1}{r}{\tt 32810}& 
\multicolumn{1}{r}{\tt 2735}& 
\multicolumn{1}{r}{\tt 71840}& 
\multicolumn{1}{r}{\tt \textbf{1489515}}  
\\ \hdashline[0.5pt/1pt]\hdashline[0.5pt/1pt]


\multicolumn{1}{l|}{min-avg}& 
\multicolumn{1}{r}{\tt 14.04}& 
\multicolumn{1}{r}{\tt 1.70}& 
\multicolumn{1}{r}{\tt 12.67}& 
\multicolumn{1}{r}{\tt 1.00}& 
\multicolumn{1}{r}{\tt 27.82}& 
\multicolumn{1}{r}{\tt 440.66} 
\\
\multicolumn{1}{l|}{max-avg}& 
\multicolumn{1}{r}{\tt 42.60}& 
\multicolumn{1}{r}{\tt 1.97}& 
\multicolumn{1}{r}{\tt 16.17}& 
\multicolumn{1}{r}{\tt 2.49}& 
\multicolumn{1}{r}{\tt 34.26}& 
\multicolumn{1}{r}{\tt 836.09} 
\\

\hdashline[0.5pt/1pt]

\multicolumn{1}{l|}{geomean-avg}& 
\multicolumn{1}{r}{\tt \textbf{18.85}}& 
\multicolumn{1}{r}{\tt 1.82}& 
\multicolumn{1}{r}{\tt \textbf{13.90}}& 
\multicolumn{1}{r}{\tt 1.16}& 
\multicolumn{1}{r}{\tt \textbf{30.43}}& 
\multicolumn{1}{r}{\tt \textbf{631.02}} 
\\

		\hline
		\multicolumn{7}{c}{\bf SPECjvm2008~\cite{specjvm2008}}\\ 	\hline
	
		
\multicolumn{1}{l|}{min-sum}& 
\multicolumn{1}{r}{\tt 30560}& 
\multicolumn{1}{r}{\tt 3832}& 
\multicolumn{1}{r}{\tt 29966}& 
\multicolumn{1}{r}{\tt 2190}& 
\multicolumn{1}{r}{\tt 65741}& 
\multicolumn{1}{r}{\tt 546396} 
\\
\multicolumn{1}{l|}{max-sum}& 
\multicolumn{1}{r}{\tt 55044}& 
\multicolumn{1}{r}{\tt 5744}& 
\multicolumn{1}{r}{\tt 45745}& 
\multicolumn{1}{r}{\tt 3480}& 
\multicolumn{1}{r}{\tt 103373}& 
\multicolumn{1}{r}{\tt 1131251} 
\\

\hdashline[0.5pt/1pt]

\multicolumn{1}{l|}{geomean-sum}& 
\multicolumn{1}{r}{\tt 33195}& 
\multicolumn{1}{r}{\tt 4142}& 
\multicolumn{1}{r}{\tt 32187}& 
\multicolumn{1}{r}{\tt 2383}& 
\multicolumn{1}{r}{\tt 70280}& 
\multicolumn{1}{r}{\tt 578408} 
\\ \hdashline[0.5pt/1pt]\hdashline[0.5pt/1pt]
		


\multicolumn{1}{l|}{min-avg}& 
\multicolumn{1}{r}{\tt 13.55}& 
\multicolumn{1}{r}{\tt 1.72}& 
\multicolumn{1}{r}{\tt 13.48}& 
\multicolumn{1}{r}{\tt 0.99}& 
\multicolumn{1}{r}{\tt 28.69}& 
\multicolumn{1}{r}{\tt 206.19} 
\\
\multicolumn{1}{l|}{max-avg}& 
\multicolumn{1}{r}{\tt 16.90}& 
\multicolumn{1}{r}{\tt 1.86}& 
\multicolumn{1}{r}{\tt 14.04}& 
\multicolumn{1}{r}{\tt 1.07}& 
\multicolumn{1}{r}{\tt 31.73}& 
\multicolumn{1}{r}{\tt 347.22} 
\\


\hdashline[0.5pt/1pt]

\multicolumn{1}{l|}{geomean-avg}& 
\multicolumn{1}{r}{\tt 14.00}& 
\multicolumn{1}{r}{\tt 1.75}& 
\multicolumn{1}{r}{\tt 13.58}& 
\multicolumn{1}{r}{\tt 1.01}& 
\multicolumn{1}{r}{\tt 29.65}& 
\multicolumn{1}{r}{\tt 244.03} 
\\


		\bottomrule
	\end{tabular}
	\caption{CK Metrics Summary: Minimum, maximum and geometric mean across the sum and 
	arithmetic mean of all loaded 
	classes 
	of a 
	benchmark suite. Bold values indicate the highest value for a metric across all 
	benchmark 
	suites.}
	\label{tab:chidamber-summary}
\end{table} 

The summarized results of the analysis are shown in \Cref{tab:chidamber-summary}.
For each benchmark suite, we report a geometric mean, the minimum, and the maximum
for the sum and for the average (arithmetic mean) of each metric across all benchmarks
of the suite.
When looking at the sums, we overall observed the highest values on five out of six
metrics on Renaissance, while the LCOM metric was the highest on ScalaBench.
With respect to the average complexity across all benchmarks of the suite,
we can see that ScalaBench has higher values than Renaissance in 5 cases.
In general we cannot say whether Renaissance is more complex than ScalaBench.
However, we see that Renaissance is in the same ball park as ScalaBench and the other suites.
The reason why Renaissance is more complex on some of the metrics is highly related to the 
number of loaded classes of the benchmark suites.
We took a look at the sum of all loaded classes across each benchmark suite and 
the number of unique loaded classes for each benchmark suite in 
\Cref{tab:chidamber-loaded-classes}.
We observed that Renaissance benchmarks on average load many classes, compared to the other 
benchmark suites.

\begin{table}[t]
	\footnotesize
	\begin{tabular}{l r r }
		\multirow{2}{*}{\bf Benchmark Suite}&  {\bf Sum All} & {\bf Sum Unique}\\
		&   {\bf Loaded Classes} & {\bf Loaded Classes}\\
		\toprule
		Renaissance		& \tt{\numprint{109004}}  & \tt{\numprint{29157}} \\
		DaCapo			& \tt{\numprint{27923}}  & \tt{\numprint{12073}} \\
		ScalaBench		& \tt{\numprint{27911}}  & \tt{\numprint{12207}} \\
		SPECjvm2008		& \tt{\numprint{50099}} &  \tt{\numprint{5274}} \\
		\bottomrule
	\end{tabular}
\caption{Loaded classes per benchmark suite.}
\label{tab:chidamber-loaded-classes}
\end{table} 


\subsection{Compiled Code Size}
\label{sec:code-size}

\input{sections/compiled-code-size}


==> sections/conclusion.tex <==
% !TEX root = ../main.tex

We presented Renaissance -- a benchmark suite consisting of 21 benchmarks
that represent modern concurrency and parallelism workloads,
written in popular Java and Scala frameworks.
To obtain these benchmarks,
we gathered a large list of candidate workloads,
both manually and by scanning an online corpus of GitHub projects.
We then defined a set of basic metrics to filter potentially interesting workloads,
and to ensure that the selection is sufficiently diverse.
Our PCA analysis revealed that the set of benchmarks selected this way
covers the metric space differently than the existing benchmark suites.
To confirm that the thus-selected benchmarks are useful,
we then analyzed them for performance-critical patterns,
which lead us to implement four new optimizations in the Graal JIT compiler.
These optimizations have a considerably smaller impact
on existing suites, such as DaCapo, ScalaBench and SPECjvm2008,
indicating that Renaissance helped in identifying new compiler optimizations.
We also identified three existing optimizations
whose performance impact is prominent.
Furthermore, by comparing two production-quality JIT compilers,
Graal and HotSpot C2,
we determined that performance varies much more on Renaissance
than on DaCapo and SPECjvm2008.

While we showed that Renaissance aids in identifying new compiler optimizations,
we believe that the suite might be beneficial for other domains as well,
such as garbage collectors, profilers, data-race detectors, and debuggers.
We leave these and other investigations to future work.


==> sections/evaluation.tex <==
% !TEX root = ../main.tex

To investigate how the new optimization opportunities
in Renaissance compare to the other suites,
we provide a comprehensive performance evaluation
that identifies the impact of each optimization discussed
in Section~\ref{sec:compiler-optimizations} on each individual benchmark.
As a consistent measure of impact across different optimizations and benchmarks,
we define the impact of an optimization as the change in the benchmark execution time
observed when the optimization is selectively disabled.
The measure thus accounts for the cumulative impact of an optimization,
including its possible (enabling or disabling)
effects on other optimizations performed by the compiler.

\begin{figure*}
\includegraphics[width=\textwidth]{experiments/performance/output-optimization-impact}
\caption{Optimization impact on individual benchmarks.
Results with black outline significant at $\alpha = 0.01$.}
\label{fig:optimization-suite-impact}
\end{figure*}

The results are summarized in Figure~\ref{fig:optimization-suite-impact}.
\forcameraready{Evaluation results shown in this section have been obtained using the G1 collector.}
More details on the experimental setup used for collecting the measurements
are described in Section~\ref{sec:appendix:charles} of the supplemental material.
The figure supports our claim
that the optimizations outlined in Section~\ref{sec:compiler-optimizations}
benefit Renaissance more than other benchmark suites -- at significance level $\alpha = 0.01$,
all (7 of 7) evaluated optimizations have an impact of at least 5\% on some Renaissance benchmark,
compared with 2 of 7 for ScalaBench, 1 of 7 for DaCapo, and 3 of 7 for SPECjvm2008.
At the same significance level, the median impact is 6.4\% for Renaissance,
compared with 2.8\% for ScalaBench, 1.8\% for DaCapo, and 3.9\% for SPECjvm2008.
\forcameraready{
In Section~\ref{sec:app:optimization-impact} of the supplemental material,
we also provide some information on how each optimization impacts the overall compilation time.
}

The architecture of Graal enables rapid development and deployment of new optimizations,
making it an obvious choice for our experiments with optimization opportunities
in modern workloads.
\forcameraready{
We found it relatively straightforward to implement new optimizations in the
open-source Graal compiler. However, if Graal were a poorly performing compiler,
the impact of each optimization relative to baseline might appear magnified. To
prove that Graal can serve as a reasonable baseline,
}
we also compared performance of the four benchmark suites on two variants of the HotSpot JVM,
one equipped with the standard C2 compiler, other with Graal, both in the role
of the final-tier compiler. The results, relative to the baseline HotSpot JVM
using the C2 compiler, are shown in \autoref{fig:graal-vs-cc}.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{../experiments/performance/output-graal-vs-cc}
\caption{Graal compiler performance relative to HotSpot second tier JIT compiler.}
\label{fig:graal-vs-cc}
\end{figure*}

% \pt{Update numbers with final data.}

Graal provides better performance than C2 in 51 out of 68 benchmarks,
the opposite is true in 10 benchmarks, for the remaining 7 benchmarks
the difference is not statistically significant as the 99\% confidence interval straddles 1.0.
On benchmarks where Graal is better than C2, the median speedup is 20\%.
On benchmarks where C2 is better than Graal, the median slowdown is 4\%.
This justifies our choice of Graal as the experimental evaluation platform.
% and ensures that we demonstrate performance impact against the performance
% of a state-of-the-art production-level compiler.

% \ap{
% I think that this section might be a good opportunity to ensure that nobody attacks us
% that we broke the double-blind review process.
% I think we might want to start with:
% "We chose to use the open-source Graal version at GitHub as a starting point
% for implementing the optimizations in the previous section."
% }
% \ap{
% I'm not sure if we should mention architecture and tooling,
% because it might sound like we're Graal devs, and we're selling it.
% Saying "open-source" might be enough, and then continuing to the question
% whether C2 is better than Graal.
% }

%The performance measurement experiments reported in this section were conducted on 8-core Intel servers\footnote{Intel Xeon E5-2620v4 CPU (2.1 GHz, 8 cores, 20 MB cache, HT disabled).}, with 64 GB RAM, running Fedora Linux 27 (kernel 4.15.6).
%For stable measurement, power management features were disabled and the processor was run at the base frequency.
%Prior to each benchmark execution, the physical memory pool was randomized.
%The virtual machine used was Oracle JDK 8u172 with Enterprise Graal 1.0.0-rc9.
%The heap size was fixed at 12 GB with the G1 collector, and except for the selection of individual compiler optimizations used to produce Figure~\ref{fig:optimization-suite-impact}, no other options were used.
%%
%For each benchmark and each optimization configuration, we have executed the measurements in a new JVM 15 times. \pt{Update this number with final data.}
%Each execution consisted of a warmup period of 5 minutes, followed by 60 seconds of measurements, rounded up to the next complete benchmark iteration.
%The duration of the warmup period was chosen so that major performance fluctuations due to compilation happen before actual measurement (verified manually).
%To provide for meaningful comparison across benchmarks, we always collect
%the execution times of the main benchmark operation (we have modified
%the SPECjvm2008 benchmark harness to achieve this, the benchmark
%would normally report aggregated throughput).
%Winsorized filtering was used to remove outliers from Figure~\ref{fig:optimization-suite-impact}.

% \ap{
% I think that we want to quantify how big the difference between Graal and C2 is on these suites.
% I.e. visually we obviously see that the smaller difference on DaCapo and SPECjvm2008.
% But how to quantify that?
% There is also a point in the introduction about this.
% }


==> sections/introduction.tex <==
% !TEX root = ../main.tex

To drive innovation in managed runtimes and just-in-time (JIT) compilers,
researchers and practitioners rely on benchmarks suites
that capture representative patterns of application behavior.
This allows developing and validating new optimizations and memory management techniques.
Even though an improvement demonstrated on a benchmark is not always a sufficient condition,
it is usually a necessary condition for a new optimization or technique to be considered useful.
The Java Virtual Machine (JVM) is at the forefront of managed runtime research and development,
and due to its popularity and widespread use,
many benchmarking suites targeting the JVM have been developed.
Of those most established, the \mbox{DaCapo} benchmark suite
introduced a set of workloads to help understand
memory behavior of complex Java applications~\cite{Blackburn:2006:DBJ:1167515.1167488}.
The \mbox{ScalaBench} suite~\cite{Sewe:2011:DCC:2048066.2048118}
focused on Scala programs, which exhibit a significantly different behavior
compared to Java programs~\cite{Sewe:2012},
despite Scala being compiled to Java bytecode and executed on the JVM.
The \mbox{SPECjvm2008} focused on computationally intensive workloads~\cite{specjvm2008},
while the more recent \mbox{SPECjbb2015} benchmark simulates the IT infrastructure
of an online supermarket~\cite{specjbb2015}.

% \ap{add a paragraph
% to reflect on the benefits that these suites brought in the past
% to motivate why benchmark suites are paramount}

% \ap{the next paragraph should ideally mention some preliminary existing proof/example
% of how an optimization was missed}

Still, as we argue in this paper,
neither of the existing benchmark suites for the JVM
was specifically focused on concurrency and parallelism.
Moreover, the JVM has evolved considerably over the years, and gained support for
atomic operations~\cite{jsr166},
% fence intrinsics~\cite{jep155}, % minor, but we did not measure, might open us to attacks ...
lock-free concurrent data structures~\cite{jep155},
and non-blocking I/O~\cite{jsr203},
as well as new language and JVM features
% \wb{
% I'd not call lambdas and a particular bytecode ``APIs''.
% Maybe better: new language and JVM features?
% }
such as Java Lambdas~\cite{jsr335},
§invokedynamic§ and method handles~\cite{jsr292}, to name a few.
At the same time, the arrival of multicore processors
prompted a plethora of new programming models and frameworks,
such as software transactional memory~\cite{Shavit:1995:STM:224964.224987,Harris:2005:CMT:1065944.1065952,Bronson10ccstm:a},
fork-join~\cite{Lea:2000:JFF:337449.337465},
data-parallel collections~\cite{jep107,Zaharia:2010:SCC:1863103.1863113,prokopec11},
and actors~\cite{akka,Srinivasan:2008:KIA:1428508.1428517,Haller:2007:AUT:1764606.1764620}.
These workloads potentially present new optimization opportunities
for compilers and virtual machines.

This paper proposes a new representative set of benchmarks
that cover modern JVM concurrency and parallelism paradigms.
While we do not argue that the proposed benchmark suite is exhaustive
in that it represents all relevant workloads or optimization opportunities,
we have found these benchmarks useful,
since they helped us identify, implement and assess new compiler optimizations.
As we show in the paper,
three other established benchmark suites did not exhibit similar characteristics.

% \wb{and ``implement and assess''?}

% \dl{
% I dont see the gap directly,
% can we repeat that with "between well established benchmark suites and
% modern concurrency focues code" ?
% }

% \ap{develop this further -- explain all contributions and claims in the paper,
% and leave the bullets below as a summary.}

The contributions in this work are as follows:

\begin{itemize}
\item
We propose a new benchmark suite,
which consists of 21 parallelism- and concurrency-oriented benchmarks for the JVM,
and relies on multiple existing state-of-the-art Java and Scala frameworks
(Section~\ref{sec:benchmarks}).
\item
We identify a set of metrics that reflect the usage
of the basic concurrency primitives on the JVM,
along with a normalization technique (Section~\ref{sec:metric-comparison}).
\item
We show that the proposed benchmarks are diverse
in the sense that they span the space of concurrency metrics better than the existing suites
(Section~\ref{sec:pca}).
\item
We demonstrate that the proposed benchmarks reveal new opportunities for JIT compilers by implementing four new optimizations in the Graal JIT compiler~\cite{Duboscq:2013:IRS:2542142.2542143} (Section~\ref{sec:compiler-optimizations}).
\item We evaluate the impact of the four new optimizations, plus three pre-existing optimizations,
on Renaissance, DaCapo, ScalaBench and SPECjvm2008 suites, showing that all 7 optimizations
exhibit over 5\% impact on Renaissance, compared to only 2 on ScalaBench, 1 on DaCapo,
and 3 on SPECjvm2008 (Section~\ref{sec:evaluation}).
\item
We show that the proposed benchmark suite is
as complex as DaCapo and ScalaBench,
and much more complex than SPECjvm2008,
by evaluating six Chidamber and Kemerer metrics,
and by inspecting the compiled code size and the hot method count of all the benchmarks
(Section~\ref{sec:complexity}),
\end{itemize}

We present related work in Section~\ref{sec:related},
and we summarize our observations in Section~\ref{sec:conclusion}.

% \wb{
% A general remark: one might accuse us of selecting benchmarks such that
% our optimizations show benefits. How shall we defend against such criticism?
% }
% \ap{
% I think there are 3 ways in which we can defend:
% 1) 14 out of 21 benchmarks were already proposed elsewhere and adopted.
% 2) All benchmarks utilize existing popular and widely-used frameworks
%    for concurrency and parallelism, not basic concurrency primitives.
% 3) We present the benchmark selection process first,
%    and say that the PCA showed us that we have a diverse selection.
%    In Section 5, we then say that,
%    having selected a satisfactory set of benchmarks according to the metrics,
%    we sought out optimizations that are relevant for those benchmarks.
% Question: is this already explicit enough in the text, or should we explicitly say it?
% }


==> sections/old-metrics-claims.tex <==
% !TEX root = ../main.tex


\subsection{Comparison with Standard Benchmark Suites}

Claims that I think we can make (based on the April 5 analysis):

...


\paratitle{Claim 1}

%\begin{figure}[t]
%\centering
%\subfigure[Renaissance]{
%\includegraphics[width=0.31\columnwidth]{figures/atomic_ren}
%}
%\subfigure[DaCapo]{
%\includegraphics[width=0.31\columnwidth]{figures/atomic_dacapo}
%}
%\subfigure[ScalaBench]{
%\includegraphics[width=0.31\columnwidth]{figures/atomic_sb}
%}
%\caption{Atomic operations.}
%
%\label{fig:fine}
%\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{../figures/atomic}
\caption{Atomic operations - Normalized by reference cycles elapsed.}
\label{fig:atomic_operations}
\end{figure}


Neither Scalabench nor Scala DaCapo use atomic operations substantially.

DaCapo best examples:

- h2 -- 1.07e-5

- jython -- 9.84e-5

- tomcat -- 6.28e-5

Scalabench best examples:

- factorie - 7.90e-5

Our best examples:

- philosophers -- 6.3e-4

- stm-bench7 -- 1.67e-4

- db-shootout -- 1.14e-4

- page-rank -- 9.56e-5

- movie-lens -- 9.93e-5

- {\sf reactors-savina} -- 7.66e-5

- akka-uct -- 1.25e-5

- rx-scrabble -- 1.36e-5

\st{
TODO(Alex): See if we can find a more realistic lmax benchmark,
since lmax really uses atomics heavily.
Investigated -- philosophers and db-shootout.
}

\paratitle{Claim 2}


\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{../figures/biasedLocks}
\caption{Kinds of locks}
\label{fig:biased_locks}
\end{figure}


Best DaCapo examples of synchronized locks are $\approx$56\%-$\approx$80\% biased,
and exhibit a smaller ratio of fast-path locks.
We have stronger examples of fast-path locking ($\approx$99\% in fj-kmeans).

Scalabench has very little synchronized blocks overall:

- specs -- 8.76e-5, $\approx$15\% biased locking, $\approx$71\% fast-path

DaCapo best examples:

- avrora -- 3.3e-5, $\approx$30\% biased, $\approx$66\% fast-path

- fop -- 1.92e-4, $\approx$79\% biased, $\approx$20\% fast-path, but 13\% CPU

- h2 -- 1e-4, $\approx$20\% biased, $\approx$42\% fast-path, but 18\% CPU

- jython -- 2.22e-4, $\approx$98\% biased, but 13\% CPU

- tomcat -- 1.15e-4, $\approx$57\% biased, $\approx$43\% fast-path

- tradesoap -- 2e-4, $\approx$56\% biased, $\approx$37\% fast-path

- xalan -- 3.7e-4, $\approx$80\% biased, $\approx$18\% fast-path

Our best examples:

- fj-kmeans -- 2.30e-3, but this is $\approx$99.75\% fast-path locking, 72\% CPU

- reactors-savina -- 1.12e-4, but this is $\approx$97\% fast-path locking, 55\% CPU

- rx-scrabble -- 1.44e-4, this is $\approx$94\% biased locking, 35\% CPU

- r5 -- 1.43e-4, this is $\approx$31\% biased, $\approx$67\% fast-path, 24\% CPU

- philosophers -- 1.2e-5, this is $\approx$33\% slow-path, and $\approx$67\% fast-path,
  93\% CPU

\st{
TODO: See if we can find a workload with more slow-path locking.
Investigated -- philosophers.
}

\st{
TODO: See if we can find a workload that is a mix of biased and fast-path.
Investigated -- we found philosophers and r5,
latter being obtained through scanning of online corpuses.
}

\st{
TODO(Alex):
See if we there is a good SnapTree benchmark that we could use
(uses synchronized and custom spin locks).
Investigated -- does not seem to be interesting.
}

\paratitle{Claim 3}
The Lock interface,
which exhibits different characteristics
compared to the synchronized statement (e.g. hand-over-hand locking pattern),
is under-represented in DaCapo and Scalabench.

This is easy to see -- DaCapo is at best in the 1e-6 range,
ScalaBench is 1e-7 and 1e-8 in two benchmarks, and 0 otherwise.

Our best examples:

- db-shootout -- 4.5e-5

- r5 -- 5.4e-6

\st{TODO: Investigate a more involved workload with MapDB and LMAX,
since micros tell us that they are good candidates.}

\st{TODO: Investigate the R5 benchmark further (e.g. is CPU usage satisfactory?).}


\paratitle{Claim 4}
While some of the benchmarks in existing suites are multi-threaded,
average CPU utilization is low.
Only a 4/12 benchmarks are heavily multithreaded (>50\%) in DaCapo,
but all our benchmarks are above $\approx$50\%,
except rx-scrabble and streaming-ads ($\approx$35\%).

Best DaCapo examples:

- lusearchfix -- $\approx$80\%, but all other concurrency metrics are low

- sunflow -- $\approx$90\%, but all other concurrency metrics are low

- tradesoap -- $\approx$64\%, but the only interesting metric is synchronization count,
  and it's $\approx$56\% biased locks

- xalan -- $\approx$97\%, but it uses $\approx$80\% biased locks

Scalabench examples:

- scalatest, factorie, kiama are $\approx$30\%, but not interesting wrt metrics

Our best examples:

- akka-uct --$\approx$~92\%

- naive-bayes -- $\approx$75\%

- fj-kmeans -- $\approx$72%

- scrabble -- $\approx$90\%

... TODO comparison ...


\paratitle{Claim 5}
Conditional monitor operations (wait/notify)
are underrepresented in existing JVM benchmark suites.

Very low in Scalabench (best are scalatest and specs with 1e-6 notify).

DaCapo avrora is 7e-6/7e-7, but the CPU utilization is only $\approx$20\%.

Our best examples:

- philosophers 8e-8/4e-7 (with $\approx$90\% CPU utilization)

- streaming-ads 2e-7 notify rate



==> sections/old-optimizations.tex <==
% !TEX root = ../main.tex


\subsection{Locking Places}
\dl{TODO}
I am not fully finished but I modified to
lock snippet counters to not only output lock kind but also
method, compilation unit and node ID, there I found patterns
that occur over some benchmarks, I am not fully done yet so maybe
somebody else can verify.


\begin{lstlisting}[language=Java]

FilterInputStream::read(byte[]):CAS
  + scrabble
  + scala stm bench
  
  Monitorenter inside a loop that is often locked
  
FilterOutputStream::write(byte[],int,int):CAS
  + R5
  
  Many single read synchronized blocks
  
  Biased Locking fails & benchmark goes into CAS
  
  
Inflater:InputStream
  + scraable
  + scala stm benchmark
  + Naive Bayes
  
URLClassPath::getNextLoader
  + scraable
  + scala stm bench
  + Naive Bayes

\end{lstlisting}


\paragraph{Example: Loop Wide Lock Coarsening}
	Implemented and proof-of-concept tested.
	Benchmark Example

\begin{lstlisting}[language=Java,caption={Loop-wide lock coarsening before},label=ls:loopwidelockcoarsening:before]
for(...){
	monitorenter(loopInvariantObject)
	... critical region ...
	monitorexit(loopInvariantObject)
}
\end{lstlisting}
\begin{lstlisting}[language=Java,caption={Loop-wide lock coarsening after},label=ls:loopwidelockcoarsening:before]
int roundTrips = 0
while(true){
	monitorenter(loopInvariantObject)
	for(...){
		... critical region ...	
		if(roundTrips > 32){
			break;
		}
		roundTrips++;
	}
	monitorexit(loopInvariantObject)
}
\end{lstlisting}
	
Question: How does these patterns happen?

Classical patterns are constructed via synchronized collections in the Java standard library like \texttt{java.util.Vector} or \texttt{synchronized.List}.
They typically synchronize on the list object itself, if a synchronized method of them is called inside a loop and the method is inlined we end up with a loop invariant lock inside a loop.
For example consider the \texttt{SynchronizedList} class in \Cref{ls:coarseningusecase}.

\begin{lstlisting}[language=Java,caption={Synchronized List},label=ls:coarseningusecase]
class SynchronizedList {
	...
	// synchronizes on the this object
	public synchronized void add(Object o){
		...
	}
	...
}

SynchronziedList foo(){
	Object[] objects = ... some source ...
	SynchronizedList l = new SynchronizedList();
	for(Object o:objects){
		l.add(o);
	}
	return l;
}

SynchronziedList fooAferInlining(){
 Object[] objects = ... some source ...
 SynchronizedList l = new SynchronizedList();
 for(Object o:objects){
	monitorenter(l)
	... critical region...
	monitorexit(l)
 }
 return l;
}
\end{lstlisting}

Happens in the FJ-KMeans benchmark:
\dl{find method where it triggers in fj-kmeans and write pattern down here}	


\paragraph{Example: Hash Code Aware Locking Snippets}
HotSpot JVM has several fast-path locking schemes. 
One of them is \emph{biased-locking} where a few bits in an objects header (called \emph{mark word} in HotSpot) are re-used for ultra fast locking.
However, if class does not define a hash code implementation (via overriding \texttt{java.lang.Object.hashCode()}) the VM reserves bits for an auto-(vm)-generated hash code
in an object's mark word.
In this case, we can no longer bias lock an object, because the header bits required for biased locking are reserved by the generated hashcode (internally called the \emph{identity hash code}).
\begin{lstlisting}[language=Java]
void foo(Object o){
	...
	System.identityHashCode(o) // we do not know if hash code is overridden
	...
	synchronized(o){
		... critical region ...
	}
}
\end{lstlisting}


\begin{lstlisting}[language=Java]
void foo(Object o){
	...
	System.identityHashCode(o) // we do not know if hash code is overridden
	...
	if(canBias(o)&&biasedLockingEnabledForClass(o)){
		biasLockObject(o)
	}else if(canCasLock(o)){
		casLock(o);
	}
	if(!locked(o)){
		slowPathLock(o);
	}
		... critical region ...	
	unlock(o) // biased, cas locked or slowpath
}
\end{lstlisting}

If the objects hashcode is set, the bias locking check can never return true, therefore it will always fail.
However, when compiling this method, we can optimize the check away as we know we will never be able to bias lock the object.
This saves a check in the fast path.



\paragraph{Example: Hash Code Aware Locking Duplication}
Building upon the previous problem, it might happen, that during compile time the compiler
cannot decide, if an object can be bias-locked, since \texttt{java.lang.Object.hashCode} is a virtual method
that can be overridden.
If class-hierarchy-analysis cannot deduce whether the method is override for a certain object (like in the example below),
Graal introduces a method load check trying to deduce if the hashcode method was overridden in an object's virtual method table.

\begin{lstlisting}[language=Java]
void foo(Object o){
	...
	o.hashCode() // we do not know if hash code is overridden
	...
	synchronized(o){
		... critical region ...
	}
}
\end{lstlisting}

In the example below, we see the vtable load and method check to see, if an object of an unknown (imprecise) type overrides
\texttt{java.lang.Object.hashCode}.
In this case, we can optimize this pattern, by duplicating a post-dominating critical region into to weaved vtable check 
\begin{lstlisting}[language=Java]
void foo(Object o){
	...
	if(o.vtable[hashCodeMethodIndex]==java.lang.Object.hashCode){
		System.identityHashCode(o)
	}else{
		o.hashCode() // overridden, perform virtual dispatch
	}
	...
	synchronized(o){
		... critical region ...
	}
}
\end{lstlisting}
After duplicating the critical region into the control flow split we can remove the bias check from the true branch.

\begin{lstlisting}[language=Java]
void foo(Object o){
	...
	if(o.vtable[hashCodeMethodIndex]==java.lang.Object.hashCode){
		System.identityHashCode(o)
		...
		synchronized(o){ // Will not try to bias lock based on the optimization above.
			... critical region ...
		}		
	}else{
		o.hashCode() // overridden, perform virtual dispatch
		...
		synchronized(o){
			... critical region ...
		}		
	}
}
\end{lstlisting}


\paragraph{Lock Profiling (potentially with speculations)}
Having profiling information for the lock paths would allow us
several things (we might sketch this in the paper as future optimizations)
\begin{itemize}
	\item Lower lock snippets early remove those paths never taken and replace with a deopt
	\item Re-order lock path strategy selection for the common case, currently we
	check (1) biased, (2) fast inflated, (3) case and (4) slowpath
	\item Earlier lowering in general exposing more opt potential to graal, 
	under the assumption unlikely lock paths will go away
\end{itemize}


\paragraph{Lock Re-Switching (Working title)}
The following pattern could probably (check JMM details) be optimized
\begin{lstlisting}[language=Java]
r = ...
monitorenter(o)
	if(r==0){
		... critical region ...
	}
monitorexit(o)
\end{lstlisting}
Optimize it to (is the comparison is not visible to other threads)
\begin{lstlisting}[language=Java]
r = ...
if(r==0){
	monitorenter(o)
		... critical region ...
	monitorexit(o)
}
\end{lstlisting}
Happens sometimes in benchmarks in a pattern that
3 of 4 branches of a switch or if cascade inside a lock
do stuff but one branch does not.
pulling the lock region into the branches could eliminate one while
the others happen normally. 


\paragraph{Lock Elimination and OSR}
OSR can prevent lock elimination.
If we have a loop locking an object before and after the loop
and the interpreter enters the lock, we will never be able to
escape analyze and remove the lock from the object if we keep an OSR
compilation of such a graph.

\paragraph{Synchronized to Re-entrant RW Lock Promotion}
Just a mind experiment started and then discussed with benoit to
think about theoretical possibility.
Sometimes code contains control flow inside locks like the following

\begin{lstlisting}[language=Java]
monitorenter(o)
	read 1
	read 2
	....
	if(...)
		write
	read ...
	read ...
monitorexit(o)
\end{lstlisting}
In the region above having a RW lock instead of the full
lock would be ok in case the write will not occur in most places.
Q is can we promote the region to automatically be a re-entrant rw lock
that only acquires a full lock if the write branch is entered ?
More like a PhD topic but ....


\vspace{5cm}
\paratitle{Example 1}
We know that vectorization and loop optimizations
helped improve Graal on data-parallel workloads (Apache Spark).

TODO: Gilles, can we find more examples in which we were able to optimize code patterns?
E.g. with respect to moniterenter/monitorexit?
Can we come up with concrete examples here?

\paratitle{Example 2}
Message-passing concurrency involves creating objects and placing them on a queue.
These objects are then picked up by the same, or another thread.
Do we see any examples where this restricts PEA from removing allocations,
and what could we do to improve PEA in these cases?

\paratitle{Example 3}
Synchronization involves writing an object to a synchronized location,
which is then read by another thread.
Similar -- can we show differences between the behaviour of standard EA and PEA?

\paratitle{Example 4}
Usage of invokedynamic -- almost none in DaCapo, but scrabble and rx-scrabble has them.
We can mention improved inlining, folding, PEA (i.e. read elimination)
as a means of eliminating them.

\paratitle{Example 5}
How do the synchronized blocks or atomics affect register allocation?


\dl{I think we could also classify all benchmarks based on their optimization potential? Either manually by inspecting the important compilation units or semi automatically with gtune?}
\ap{How do you suggest we measure optimization potential? E.g. try different parameters and see if they improve performance?}
\dl{Yes, find the 5 most important optimizations (besides canonicalization \& inlining which will be important for every benchmark) but besides that.
	Knowing which transformations are performance relevant already gives a lot of insight for further optimizations and improvements}


\medskip

\dl{I think a big part of the contribution would also be the benchmark suite itself so it can be used by other researchers and compilers therefore we should also do the artifact evaluation track if possible 
	and we should be able to show a reproducability for all those numbers an claims, meaning they should be easily repeatable, at least the performance numbers
}
\ap{Agreed. Petr Tuma's group will be working on publishing the suite in the open source....
}


\medskip

\dl{
	For reproducability we would need
		+ docker images building stuff (like graal) , Q: how to get enterprise automatically downloaded (e.g. graalvm)?
		+ scripts to run the benchmarks
		+ same scripts we use in the paper to get performance nrs
}


==> sections/optimizations.tex <==
% !TEX root = ../main.tex


% \ap{
% Each optimizations should have:
% (1) a concise description of the pattern,
%     if necessary with a code and/or a benchmark/code reference
% (2) a concise code example or a simple IR figure
% (3) a concise explanation of the optimization
% (4) a small performance plot with and without the optimization,
%     showing impact on the respective benchmark
% }

% \wb{
% In some snippets you show pseudo-code, in others you show Java code.
% You could try to unify the code style in the snippets,
% or make it explicit when referring to pseudo-code.
% }

Once we identified a sufficiently diverse set of benchmarks,
as explained previously in Sections \ref{sec:benchmarks},
\ref{sec:metric-comparison} and \ref{sec:pca},
we wanted to check if these benchmarks help us
in identifying new optimization opportunities.
We therefore investigated if we can develop new JIT-compiler optimizations
that are useful for the code patterns that appear in Renaissance benchmarks.

In this section, we analyze several compiler optimizations
for which we noticed a significant impact on Renaissance benchmarks,
and we explain the reason for the impact.
For the purposes of the analysis,
we used the Graal JIT compiler to implement 4 new optimizations\footnote{
  Graal's compliance test suite is available at GitHub~\cite{github-jtt},
  and we ran it to check that our implementations are correct.
}
(escape analysis with atomic operations, loop-wide lock coarsening,
atomic-operation coalescing, and method-handle simplification),
and to study 3 existing optimizations
(speculative guard movement, loop vectorization, and
dominance-based duplication simulation).
Notably, we do not claim that these are the only optimizations
that are important for the Renaissance benchmarks --
we only discuss those parallelism-related optimizations that we were able to identify.
\forcameraready{
Also, we focused on high-level optimizations
for the existing backends of the Graal compiler.
In particular, we did not study fence optimizations although they are interesting for
platforms such as PowerPC or AArch64\footnote{
\forcameraready{
Graal has no PowerPC backend that we know of and its AArch64 backend
has not yet been optimized for fine-grained use of fences.
}}.
}

In the rest of the section, we briefly explain each optimization and
discuss its impact on the benchmarks.
We also establish a relationship to the metrics from Section~\ref{sec:metric-comparison}
and illustrate performance with data cited from Section~\ref{sec:evaluation}.
We present a minimal example for each optimization --
while such examples are rare in the source code,
they do appear in the compiler after transformations such as inlining.

\forcameraready{
In sections where optimization soundness is not apparent, we reason as follows.
Each program $P$ has some set $R$ of possible results,
where a result is a sequence of external side-effects that the program's threads make.
An external side-effect is an output of the program that the user can observe
(for example, the exit status or the I/O).
Program's executions can produce different results because
the program-threads' execution schedule is non-deterministic.
When writing a concurrent program, users consider the program correct
if its executions produce some result from the set of allowed results $R$.
However, users are not allowed to assume
any probability distribution of the program's results across executions.
Thus, for an optimization to be valid,
it must transform an original program $P$ with a set of possible results $R$
into a program $P'$ with a set of possible results $R'$,
such that $R' \subseteq R$.
For each optimization, we informally reason why the set of results of the transformed program
is either equal to that of the original program or its strict subset.
}


\subsection{Escape Analysis with Atomic Operations}

Partial Escape Analysis (PEA)~\cite{Stadler:2014:PEA:2581122.2544157}
is an optimization that reduces the amount of object allocations
by postponing heap allocation of an object until it escapes and can be seen by other threads.
PEA does this by analyzing the reads and writes to the allocated objects.
So far, the PEA in Graal was limited to regular reads and writes,
but it did not consider atomic operations such as Compare-And-Swap (CAS).

\setlength{\columnsep}{0pt}
\begin{wrapfigure}{r}{4.1cm}
\vspace{-0.2cm}
\begin{minipage}{4.5cm}
\vspace{-0.2cm}
\begin{lstlisting}[
  language=java,
  label=list:vcas,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=left,
  numbersep=2pt,
]
o = new A(v);
CAS(o.x, v, new B(v2));
CAS(o.x.y, v2, v3)
return o.x;
\end{lstlisting}
\end{minipage}
\vspace{-0.5cm}
\end{wrapfigure}
Consider the example on the right:
if the §CAS§es are not accounted for during PEA,
then the §A§ and §B§ objects must be allocated before the first §CAS§.

A CAS operation involves up to three objects:
the object containing the field, the expected value and the new value.
If the object containing the field has not yet escaped,
the CAS can simply update the state of the scalar-replaced object.
This might replace the two other objects with scalars.
This also helps when the objects escape later, because the CAS operation can be removed
and the objects can be directly initialized in their mutated state before being published.
In particular, this initialization can be performed
with---potentially cheaper---regular writes rather than with atomic instructions.

\begin{wrapfigure}{r}{3.8cm}
\vspace{-0.3cm}
\hspace{-0.26cm}
\begin{minipage}{3.8cm}
\begin{lstlisting}[
  language=java,
  label=list:vcas-after,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=none,
  numbersep=2pt,
]
return new B(v3);
\end{lstlisting}
\end{minipage}
\vspace{-0.5cm}
\end{wrapfigure}
For example, in the previous code, assuming the constructors don't let the objects escape,
the allocation of the §A§ object can be completely eliminated
and the value of the field in the §B§ object can directly be set to its updated value (§v3§).
%\wb{Is this really the case? You're assuming that A and B are not escaping from their constructors. This seems to be a necessary precondition for the optimization to be valid.}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/atomic.pdf}
\caption{Number of \metric{atomic} operations executed, normalized by reference cycles.}
\label{fig:atomics}
\end{figure}

We observed this pattern in usages of §java.util.Random§,
§com.twitter.util.Promise§, and §java.util.concurrent.atomic.AtomicReference§.
These classes change their internal state using a §CAS§ operation.
An application can create an instance of these classes and change its internal state
a few times before discarding it (full escape analysis),
or publishing it to the rest of the program (partial escape analysis).

% \begin{wrapfigure}{r}{0.125\textwidth}
% \vspace{-0.2cm}
% \begin{minipage}{4cm}
% \input{experiments/virt-cas}
% \end{minipage}
% \vspace{-0.5cm}
% \end{wrapfigure}
This optimization has a $24\%$ impact on \bench{finagle-chirper}.
As seen in Figure~\ref{fig:atomics}, this benchmark exhibits a higher value
for the \metric{atomic} metric than any of the benchmarks from the existing suites.
This is coherent, since the optimization targets
an operation counted by the \metric{atomic} metric.

\forcameraready{
\paratitle{Soundness} Objects that have not yet escaped
cannot be observed or mutated by other threads by definition. Consequently, any schedule of the
original program $P$ will yield the same outcome for the CAS operation: the transformed program
$P'$ emulates this behavior on the thread which executed the CAS in $P$. If the object
containing the memory location subject to CAS can be entirely escape-analyzed away in $P'$, no
other thread can observe the effects of this CAS in $P$. In this case, $P'$ does not contain any
external side-effect for this CAS and any result of $P'$ is a possible result of $P$. If the
object escapes at a later point in the program, its fully initialized state containing the
emulated effects of the CAS is safely published during the side-effect that causes the object to
escape. In this case any schedule of $P'$ can be mapped to a schedule of $P$ where all
side-effects due to the initialization of this object happened before the escape point.
}


\subsection{Loop-Wide Lock Coarsening}

\setlength{\columnsep}{0pt}
\begin{wrapfigure}{r}{0.2\textwidth}
\vspace{-0.4cm}
\begin{minipage}{4cm}
\begin{lstlisting}[
  language=java,
  label=list:for-sync,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=left,
  numbersep=2pt,
]
for(;condition;)
  synchronized(x) {
    ... region ...
  }
\end{lstlisting}
\end{minipage}
\vspace{-0.4cm}
\end{wrapfigure}
Consider the Java loop shown in the snippet
on the right enclosing a §synchronized§ statement,
which protects a critical region.
The time spent entering and exiting the critical region
can critically affect performance if the loop is frequently executed.

\setlength{\columnsep}{0pt}
\begin{wrapfigure}{l}{0.22\textwidth}
\vspace{-0.5cm}
\hspace{-0.5cm}
\begin{minipage}{4cm}
\begin{lstlisting}[
  language=java,
  label=list:for-sync-for,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=left,
  numbersep=2pt,
]
int b = 0;
for (;condition;)
  synchronized(x) {
    for(;condition;) {
      ... region ...
      b++;
      if (b % T == 0)
        break; } }
\end{lstlisting}
\end{minipage}
\vspace{-0.3cm}
\end{wrapfigure}
This synchronization pattern occurs when accessing
synchronized collections such as the JDK §java.util.Vector§ and §SynchronizedList§
(whose operations use locks~\cite{openjdk-vector,openjdk-synclist})
inside a loop.

To reduce the cost of locking and unlocking within the §synchronized§ block,
we extended Graal with an optimization that coarsens the lock~\cite{diniz1998lock}
by tiling the iteration space
into $C$-sized chunks, as seen in the second snippet.
The lock is held in the entire nested loop,
so the total number of monitor operations decreases.
The necessary condition is that the code motion on §condition§ and §region§ is legal
(e.g., §condition§ must not obtain another lock).

\forcameraready{
Existing lock optimizations in HotSpot's C2~\cite{Paleczny:2001:JHT:1267847.1267848} compiler
can optimize loops that have a statically known number of iterations,
by completely unrolling and coarsening the lock across the unrolled iterations.
By contrast, our optimization tiles the iteration space of any loop to
coarsen the lock, without pulling the lock out of the loop completely.
Lock coarsening has an effect on fairness,
but since \texttt{synchronized} regions in Java are inherently not fair,
this optimization does not change the program semantics --
applications relying on fairness must anyway use more elaborate locking mechanisms,
such as the §ReentrantLock§ class from the JDK.
}

% \setlength{\columnsep}{0pt}
% \begin{wrapfigure}{r}{0.125\textwidth}
% \vspace{-0.6cm}
% \begin{minipage}{4cm}
% \input{experiments/loop-wide-lock-coarsening}
% \end{minipage}
% \vspace{-0.5cm}
% \end{wrapfigure}
Loop-wide lock coarsening improves \bench{fj-kmeans} by about $71\%$.
We found that a chunk size of $C = 32$ works well for this benchmark.
Generally, the impact depends on the size of the critical region,
as well as the number of loop iterations.
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/synch.pdf}\\
% \includegraphics[width=\columnwidth]{figures/synch_alt}
\caption{Number of synchronized methods or blocks executed, normalized by reference cycles.}
\label{fig:synch}
\end{figure}
Figure~\ref{fig:synch} shows the synchronization counts across the suites,
normalized by the CPU reference cycles.
Note that ¡fj-kmeans¡ uses the §synchronized§ primitive considerably more often,
which made it possible to identify this optimization.

\forcameraready{
\paratitle{Soundness}
Any schedule $s'$ of the transformed program $P'$
can be mapped to a schedule $s$ of the original program $P$,
such that the respective external side-effects $r'$ and $r$ are equal.
Consider a schedule $s'$ of $P'$ in which some thread $T$ is about to execute
a loop that contains a synchronized region,
and which has external side-effects $r_0$
and the memory state $m_0$ before executing that loop.
There exists some execution schedule $s$ of $P$
in which all other threads pause during the execution of the $C$ iterations of the loop.
That execution schedule has the same external side-effects $r_0$
and the memory state $m_0$ before executing that loop.
Since §condition§ does not acquire any locks,
it is easy to show that both $s$ and $s'$ have the same set of external side-effects
and the same memory state after executing $C$ iterations of the loop.
By induction, the two execution schedules have the same external side-effects $r' = r$,
so the transformation is correct.
}


\subsection{Atomic-Operation Coalescing}
\setlength{\columnsep}{0.0pt}
\begin{wrapfigure}{r}{0.215\textwidth}
\vspace{-0.4cm}
\begin{minipage}{5cm}
\begin{lstlisting}[
  label=list:cas-cas,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=left,
  numbersep=2pt,
]
do {
  v = READ(x)`\label{code:cas-cas-read-1}`
  nv = f1(v)
} while(!CAS(x,v,nv))`\label{code:cas-cas-cas-1}`
do {
  v = READ(x)`\label{code:cas-cas-read-2}`
  nv = f2(v)
} while(!CAS(x,v,nv))`\label{code:cas-cas-cas-2}`
\end{lstlisting}
\end{minipage}
\vspace{-0.4cm}
\end{wrapfigure}
A typical retry-loop in lock-free algorithms
reads the value at a memory address,
and uses a §CAS§ instruction to atomically replace the old value
with the newly computed value.
If the §CAS§ fails due to a concurrent write by another thread, the loop repeats,
or otherwise terminates.
The code snippet on the right shows two such consecutive retry-loops.
\forcameraready{
This pattern rarely appears directly in user programs,
but it does occur after inlining high-level operations,
such as random-number generators or concurrent counters.
}

Consider an execution schedule in which no other thread makes progress
between the §READ§ in line \ref{code:cas-cas-read-1}
up to the §CAS§ in line \ref{code:cas-cas-cas-2},
In this execution schedule,
the intermediate §CAS§ in line \ref{code:cas-cas-cas-1}
is not observed by any other thread.
\forcameraready{
According to the Java Memory Model~\cite{jsr133},
threads are not guaranteed to observe other execution schedules of this snippet,
so user programs should not assume that they will ever see §f1(v)§.
}

\setlength{\columnsep}{0pt}
\begin{wrapfigure}{l}{0.22\textwidth}
\hspace{-0.5cm}
\begin{minipage}{4.0cm}
\vspace{-0.4cm}
\begin{lstlisting}[
  language=java,
  label=list:cas-cas-loop,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=left,
  numbersep=2pt,
]
do {
  v = READ(x)
  nv = f2(f1(v))
} while(!CAS(x,v,nv))`\label{code:cas-transformed-cas-1}`
\end{lstlisting}
\end{minipage}
\vspace{-0.4cm}
\end{wrapfigure}
Consequently, if the functions §f1§ and §f2§ are referentially transparent,
the new value §nv§ of the first §CAS§ can be directly replaced
with the new value §nv§ of the second §CAS§,
and the second §CAS§ can be removed;
the resulting snippet is on the left.

% \ap{Removing this paragraph, because it will be too complicated for the reviewers}
% More generally, this optimization starts at an initial §CAS§,
% and follows the control flow.
% If it encounters a memory access to the same address as the initial §CAS§,
% or any final-field read,
% then the corresponding expression for that address is recorded.
% If it encounters a control-flow branch,
% it checks if the condition is constant given the recorded values,
% and follows the corresponding branch.
% Upon reaching any other statement,
% the optimization replaces the new value of the initial §CAS§
% with the last recorded expression at that address.
% Other encountered writes (to the same address) are removed.

% \setlength{\columnsep}{0pt}
% \begin{wrapfigure}{r}{0.125\textwidth}
% \vspace{-0.2cm}
% \begin{minipage}{4cm}
% \input{experiments/atomic-operation-coalescing}
% \end{minipage}
% \vspace{-0.5cm}
% \end{wrapfigure}
We observed this pattern in §java.util.Random§ usages,
where the method §nextDouble§ consecutively executes a §CAS§ twice.
This optimization mostly affects ¡future-genetic¡,
improving it by $\approx$$24\%$.
The high atomic operations rate in ¡future-genetic¡,
shown previously in Figure~\ref{fig:atomics},
is due to the shared use of a pseudo-random generator,
and this optimization reduces the overall contention by eliminating some §CAS§es.

\forcameraready{
\paratitle{Soundness}
Call the original program $P$, and the transformed program $P'$.
Let $S$ be the subset of all the execution schedules of $P$
in which some thread $T$ executes the §CAS§ instructions
in lines \ref{code:cas-cas-cas-1}-\ref{code:cas-cas-cas-2},
during which all other threads are paused.
We will show that any schedule of $P'$ can be mapped to $s \in S$.

First, consider some schedule $s'$ of $P'$
in which the §CAS§ in line \ref{code:cas-transformed-cas-1} succeeds.
There must exist an execution schedule $s \in S$ of $P$
that is exactly the same as $s'$
until the lines \ref{code:cas-cas-cas-1}-\ref{code:cas-cas-cas-2}.
Before $T$ executes the §CAS§ in line \ref{code:cas-transformed-cas-1} of $P'$,
the set of external side-effects must have been $r_0$ in both $s$ and $s'$,
and the state of the memory must have been $m_0 \cupdot \{ $§x§$ \rightarrow $§v§$ \}$.
After $T$ executes the §CAS§ in line \ref{code:cas-transformed-cas-1} of $P'$,
external side-effects remain $r_0$ because §f1§ and §f2§ are referentially transparent,
and memory state becomes $m_0 \cupdot \{ $§x§$ \rightarrow $§f2(f1(v))§$ \}$.
Since the §CAS§ in line \ref{code:cas-transformed-cas-1} of $P'$ succeeds in $s'$,
then §CAS§ in line \ref{code:cas-cas-cas-1} of $P$ succeeds in $s$.
Since $s \in S$, the §CAS§ in line \ref{code:cas-cas-cas-2} must also succeed.
Consequently, after $T$ executes
the lines \ref{code:cas-cas-cas-1}-\ref{code:cas-cas-cas-2} of $P$,
the set of external side-effects is $r_0$,
and $m_0 \cupdot \{ $§x§$ \rightarrow $§f2(f1(v))§$ \}$ is the state of the memory.

Therefore, in the schedule $s \in S$, after the other threads resume,
$P$ has the same memory state as $P'$ in $s'$,
so the remaining external side-effects $r_1$ must be the same in both $s$ and $s'$,
and the execution has the same result $r' = r = r_0 \cdot r_1$.
The proof is similar when the §CAS§ in line \ref{code:cas-transformed-cas-1} of $P'$ fails.

In conclusion, any schedule $s'$ of $P'$ can be mapped
to some schedule $s$ in $P$ that has the same result $r = r'$.
By the previous definition, $R' \subseteq R$ and the transformation is correct.
}


\subsection{Method-Handle Simplification}

Java~8 Lambdas are used to express declarative operations
in multiple frameworks such as Java Streams~\cite{jep107},
futures~\cite{jsr166,jep155,jep266,github-finagle}, and Rx~\cite{rx}.
In the bytecode, the lambda-value creation is encoded
with an §invokedynamic§ instruction~\cite{jsr292}.
The first time this instruction is executed,
a special \emph{bootstrap method} generates an anonymous class for the lambda,
and returns a \emph{method handle}.
The method handle's §invoke§ method is then used to call the lambda.

\setlength{\columnsep}{0pt}
\begin{wrapfigure}{l}{0.19\textwidth}
\hspace{-0.8cm}
\vspace{-0.5cm}
\begin{minipage}{4.0cm}
\vspace{-0.6cm}
\begin{lstlisting}[
  language=java,
  label=list:invoke-dynamic,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=none,
  numbersep=2pt,
]
...
invokedynamic #14, 0
aload 11
invokevirtual #15, 2
...
\end{lstlisting}
\end{minipage}
\end{wrapfigure}
Consider the sequence of bytecodes shown on the left.
By the time this code gets compiled,
the §invokedynamic§ gets replaced with the address
of the generated method-handle object.

\setlength{\columnsep}{4pt}
\begin{wrapfigure}{r}{0.14\textwidth}
\hspace{-0.0cm}
\vspace{-0.4cm}
\begin{minipage}{4.0cm}
\vspace{-0.4cm}
\includegraphics[scale=0.07]{../figures/method-handle-invoke.pdf}
\end{minipage}
\end{wrapfigure}
The figure on the right shows the corresponding program segment
in the intermediate representation
used by Graal~\cite{Duboscq:2013:IRS:2542142.2542143}.
The §Invoke§ node represents the second invoke,
while §Arguments§ encapsulates the argument list.
Importantly, the first argument §C§ is a constant
that represents the address of the method-handle in memory.

In frameworks that parameterize operations with lambda values,
inlining the body of the lambda typically triggers other optimizations.
Unfortunately, the method handle's §invoke§ method is polymorphic,
which prevents the inlining.
% To enable inlining, method-handle calls
% must be converted to calls with known targets.
Even though the method-handle object has a constant address, the compiler does not know
\emph{the actual code of the JVM method that the method-handle object refers to}.
We therefore used the existing JVM compiler interface~\cite{jep243}
% \wb{Does this statement break the double-blind reviewing policy?}
% \ap{Rephrased to "used the existing" instead of "extended".}
to resolve the method-handle-object address
to the JVM method that is encapsulated within the method handle.
This allowed us to replace method-handle calls with direct calls,
which can be inlined in the subsequent phases in the compiler.

We found that this generally improves performance across multiple methods.
For example, using Oracle Developer Studio~12.6,
we recorded the hottest methods in ¡scrabble¡,
along with the execution times with and without this optimization.

\noindent
{
\setlength{\tabcolsep}{3.5pt}
\footnotesize
\begin{tabular}{R{0.7cm} R{0.7cm} L{6.4cm}}
\toprule
{\bf with (ms)} & {\bf w/o (ms)} & {\bf Compilation unit} \\
\midrule
\num{303.4}     & \num{350.0}    & <Total> \\
\num{25.9}     &  \num{29.6}    & §JavaScrabble.lambda\$run\$2§ \\
\num{23.7}     &  \num{23.1}    & §java.util.Spliterator\$OfInt.forEachRemaining§ \\
\num{22.4}     &  \num{28.8}    & §java.util.stream.ReferencePipeline\$3\$1.accept§ \\
\num{18.1}     &  \num{20.4}    & §JavaScrabble.lambda\$run\$5§ \\
% ...      &  ...     & ... \\
\bottomrule
\end{tabular}
}

\forcameraready{
In the preceding table,
method-handle simplification reduces the execution time for most methods,
but not for the §forEachRemainining§ method of the §Spliterator§ interface.
The reason is as follows: parallel Stream operations split collections into subsets,
pass some subsets to worker threads, and some to the calling thread.
The §invokedynamic§ instruction that creates the method-handle
is executed on the calling thread.
Thus, the method-handle type can be statically determined on the calling thread,
but not on the worker threads, which invoke the §forEachRemaining§ method.
This indicates additional opportunities for optimizations in the future.
}

\setlength{\columnsep}{0pt}
\begin{wrapfigure}{l}{0.225\textwidth}
\hspace{-0.5cm}
\vspace{-0.45cm}
\begin{minipage}{4.0cm}
\vspace{-0.6cm}
\begin{lstlisting}[
  language=java,
  label=list:scrabble-pattern,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=left,
  numbersep=2pt,
]
histogram = word ->
  word.chars().boxed()
    .collect(groupingBy(
      identity(),
      counting()));
\end{lstlisting}
\end{minipage}
\end{wrapfigure}
Method §lambda\$run\$2§ corresponds to the Java code on the left:
a lambda that produces a histogram of characters for a given string.
Using Graal, we inspected the intermediate representation of this method,
both with and without the optimization.
The additional inlining induced by method-handle simplification
triggers other optimizations that reduce the number of callsites from 19 to 1,
remove 37 out of 61 dynamic type- and null-checks,
and reduce the total number of IR nodes in that method from 696 to 490.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/invoke.pdf}
\caption{Number of {\tt invokedynamic} bytecodes executed, normalized by reference cycles.}
\label{fig:idynamic}
\end{figure}

Overall, method-handle simplification impacts the running time
of ¡finagle-chirper¡ by $4\%$,
¡scrabble¡ by $22\%$,
¡streams-mnemonics¡ by $7\%$,
and ¡rx-scrabble¡ by $1\%$.
These results correlate with
the §invokedynamic§ counts normalized by CPU reference cycles,
shown in Figure~\ref{fig:idynamic}.
On \mbox{DaCapo}, \mbox{ScalaBench}, and \mbox{SPECjvm2008}
(which precede §invokedynamic§),
the calls to §invokedynamic§ usually occur only indirectly through the Java class library.
%when invoking a JDK API.


\vspace{0.4cm}
\subsection{Speculative Guard Motion}

\begin{wrapfigure}{r}{3.9cm}
\vspace{-0.4cm}
\begin{minipage}{4.5cm}
\begin{lstlisting}[
  language=java,
  label=list:guard-motion,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=left,
  numbersep=2pt,
]
for (i=0; i<N; i++) {
  if (...) {
    guard(0<=i<L);
    ...
  }
}
\end{lstlisting}
\end{minipage}
\vspace{-0.5cm}
\end{wrapfigure}
JIT compilers for the JVM often use speculative optimizations.
Some of these optimizations require the insertion of \emph{guards},
which ensure the speculation is correct at runtime.
If the speculation is not correct, these guards divert the execution
to an environment that does not use speculations (i.e., an interpreter, or code compiled by a baseline compiler).
New profiling then takes place and a re-compilation that does not use the respective speculation is triggered.
In order to avoid useless re-compilations,
guards are not typically hoisted out of the branch where they are needed.

\begin{wrapfigure}{l}{4.0cm}
\vspace{-0.5cm}
\hspace{-0.5cm}
\begin{minipage}{4.2cm}
\begin{lstlisting}[
  language=java,
  label=list:guard-motion-after,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=left,
  numbersep=2pt,
]
guard(0<L && 0<=N-1<L);
for (i=0; i<N; i++) {
  if (...) {
    ...
  }
}
\end{lstlisting}
\end{minipage}
\vspace{-0.5cm}
\end{wrapfigure}
However, for some loops, it is beneficial to speculatively hoist guards out of loops
even if the control-flow in the loop does not always lead to that guard.
This is beneficial because the hoisted guards are executed less often.
To capture typical cases such as bounds checks,
comparisons of induction variables can be rewritten to loop-invariant versions.
Speculative Guard Motion is described in more details by~\citet{duboscq-thesis}.
This optimization has a $15\%$ impact on the \bench{log-regression} benchmark
and an $8\%$ impact on the \bench{dec-tree} benchmark.
To better understand this difference, we measured the number of guards executed
with and without speculative guard motion for the \bench{log-regression} benchmark.

% \wb{Consider using numprint for all measurement numbers in the paper.}

\begin{center}
\setlength{\tabcolsep}{3.5pt}
\footnotesize
\begin{tabular}{r r l}
 \toprule
 \multicolumn{2}{c}{\bf Executions} & {\bf Guard type} \\
 \midrule
 \multicolumn{3}{c}{\bf Without} \\
 \midrule
          \num{57487131} &   \num{1}\% & Others                 \\
         \num{529958424} &  \num{10}\% & §UnreachedCode§        \\
       \num{1639903998} &  \num{32}\% & §NullCheckException§   \\
       \num{2917610059} &  \num{57}\% & §BoundsCheckException§ \\
 \hdashline[0.5pt/1pt]
       \num{5144959612} & \num{100}\% & Total                  \\
 \midrule
 \multicolumn{3}{c}{\bf With} \\
 \midrule
          \num{55660483} &   \num{7}\% & Others                                    \\
          \num{18314637} &   \num{2}\% & \emph{Speculative} §NullCheckException§   \\
          \num{22056283} &   \num{3}\% & \emph{Speculative} §UnreachedCode§        \\
          \num{28570247} &   \num{3}\% & \emph{Speculative} §BoundsCheckException§ \\
          \num{62046637} &   \num{7}\% & §BoundsCheckException§                    \\
         \num{166341946} &  \num{20}\% & §NullCheckException§                      \\
         \num{499933160} &  \num{59}\% & §UnreachedCode§                           \\
 \hdashline[0.5pt/1pt]
         \num{852923393} & \num{100}\% & Total                                     \\
 \bottomrule
\end{tabular}
\end{center}

First, note that the total number of executed guards is reduced by $83\%$.
Moreover, note the entry for \emph{speculative} guard variants,
which accounts for the hoisted guards.
In particular, we can see the large effect on
§BoundsCheckException§ and §NullCheckException§ guards where most occurrences have been replaced by the lower-frequency speculative versions.

In some cases, removing the guards enables additional optimizations.
Loop vectorization, discussed next, is one such example --
we found that by disabling speculative guard motion,
loop vectorization almost never triggers.
% This is due to the fact that loops containing guards cannot be vectorized.
% \ap{Explained in the next section}

\forcameraready{
\paratitle{Soundness} Hoisting guards of loop-invariant conditions is sound since executing unnecessary guards is always sound: guards have no external side-effects, they only run the risk of reducing performance.
In this case performance is conserved by not doing this transformation again if a deoptimization already happened for this loop.
The rewrite of loop-variant inequalities ($<$, $>$, $\leq$, $\geq$, signed and unsigned) involving loop induction variables requires the induction variable to change monotonically which can be statically or dynamically checked above the loop.
Once this is established, if the inequality holds at both bounds, it holds over the whole range.
As a result, the hoisted guard implies the original one, ensuring the transformed program will deoptimize in at least as many cases as the original.
}

\subsection{Loop Vectorization}

% Vectorization is a compiler technique that transforms
% sequential scalar computations into a single simultaneous vector operation,
% and is often backed by CPU instructions.
% These instructions are categorized as ¡Single Instruction, Multiple Data¡ (SIMD).
% Applications can benefit from vectorization
% by exploiting data parallelism at instruction level.
% In other words, programmers can achieve automatically a factor of performance improvement
% up to the size of vector supported by underlying hardware.

Modern CPUs include vector instruction sets that ensure better performance
by operating on multiple memory addresses at once~\cite{avx-blog}.
Most languages do not have dedicated abstractions for these instructions,
so the compiler transforms parts of the program to use vector instructions,
when possible.

\setlength{\columnsep}{0pt}
\begin{wrapfigure}{r}{0.22\textwidth}
\hspace{-0.5cm}
\vspace{-0.0cm}
\begin{minipage}{4.4cm}
\vspace{-0.1cm}
\begin{lstlisting}[
  language=java,
  label=list:vect-sum,
  captionpos=t,
  abovecaptionskip=-\medskipamount,
  numbers=left,
  numbersep=2pt,
]
for(i=0; i<N; i++) {
  c[i] = a[i] + b[i];
}
\end{lstlisting}
\end{minipage}
\end{wrapfigure}
Consider a simple Java loop shown on the right.
When separate loop iterations have no data dependencies,
a compiler can aggregate arithmetic operations from several consecutive iterations
into a single vector operation.
However, on the JVM, the code must also perform a bounds check on each array access,
which introduces additional guards into the loop, and normally prevents vectorization.
Speculative guard motion makes loop vectorization possible,
since it moves the bounds-check guards outside of the loop.

We found that combining loop vectorization with speculative guard motion
results in a $\approx$$10\%$ impact on ¡als¡,
and a $\approx$$3\%$ impact on ¡dec-tree¡.

% \ap{Old version below we decided to comment out, and shorten.}

% Vectorization is particularly applicable on loops with array accesses.
% Consider the trivial Java loop on the right.
% If there is no data dependency between one loop iteration and its preceding iteration
% (which is obvious in this case), the compiler can aggregate arithmetic operations
% from different loop iterations into a single virtual vector operation,
% e.g., $c[0:N]=a[0:N]+b[0:N]$ \yz{commonly used?}.\gd{i think that's a good simple example}
% Depending on the supported vector size,
% the compiler will then segment the virtual vector operation
% into multiple or looped SIMD instructions.
% \yz{
% I believe this is what we do in Graal, correct me if wrong.
% C2 would first perform unroll and then aggregate operations within a single iteration.
% Even though there could be data dependency between different unrolled iteration,
% C2 is still able to perform vectorization.
% }
% \gd{yes, what we describe here is loop vectorization, not ``SIMD vectorization''}

% Yet, JVM needs to perform boundary check upon each array access,
% as per the Java language specification.
% This introduces additional control flow within the loop body, and disturbs vectorization.
% Thanks to the ¡Speculative Guard Motion¡ optimization,
% the compiler is able to hoist such checks,
% leaving only the arithmetic operations in the loop body, and thus re-enables vectorization.

% We found that vectorization has a significant
% impact on performance across different Renaissance workloads.
% Take ¡AlternatingLeastSquares¡ as example,
% one particular loop~\cite{github-als},
% which performs $float$ to $double$ conversion iteratively on array element,
% dominates the running time.
% By turning on vectorization, we are able to achieve \yz{20\%} performance improvement.
% As a side note, disabling ¡Speculative Guard Motion¡ optimization
% completely shuts down the speedup by vectorization.

% The concept of vectorization is not new.
% Yet a vectorization-applicable benchmark suite is essential to compiler writers,
% because of the new CPU features being developed.
% For example, Intel has been pushing its latest vector extension set
% AVX512\footnote{https://software.intel.com/en-us/blogs/2013/avx-512-instructions}.
% This extension not only enables 512-bit ZMM registers that allow
% 16 simultaneous arithmetic operations of 32-bit integers, but also brings new features,
% such as gather-scatter operations for vector addressing.

% https://yankee.ms.mff.cuni.cz/work/2018-11-14/plot-overview.nb.htmlThese new features await compiler writers to base their optimization implementation on,
% and to conduct thorough evaluation.
% Only if the performance impact of such features is validated by real-world applications,
% the compiler then may switch corresponding optimizations on by default.
% For example, Intel contributed a reduction vector optimization to
% OpenJDK\footnote{https://bugs.openjdk.java.net/browse/JDK-8074981},
% and was later restricted
% because of performance regression\footnote{https://bugs.openjdk.java.net/browse/JDK-8078563}.

% We believe there are other vectorization opportunity by involving new CPU features.
% To this end, we have selected various modern workloads whose data model are
% vectorization friendly, such as \yz{xxx, yyy, zzz}.
% Specially, the \yz{workload placeholder} employs a common code pattern that
% corresponds to nowadays streaming API usage.
% Once inlining reduces such code patterns into simple loops,
% the vectorization will kick in and accelerate applications by exploiting data parallelism.


\subsection{Dominance-Based Duplication Simulation}

\begin{wrapfigure}{r}{0.24\textwidth}
\vspace{-0.5cm}
\hspace{-0.15cm}
\begin{minipage}{4.2cm}
\vspace{-0.0cm}
\begin{lstlisting}[
  language=java,
  label=list:duplication-typecheck-opportunity,
  captionpos=t,
  numbers=left,
  numbersep=2pt
]
if (x instanceof C) a()
else b()
if (x instanceof C) c()
\end{lstlisting}
\end{minipage}
\vspace{-0.5cm}
\end{wrapfigure}
Dominance-\-based duplication simulation (DBDS)~\cite{Leopoldseder:2018:DDS:3179541.3168811}
is an optimization that simplifies control flow
by duplicating the code after control-flow merges.
Consider the pattern on the right,
which consists of two subsequent §instanceof§-checks
on the same class §C§.

\begin{wrapfigure}{l}{0.22\textwidth}
\vspace{-0.5cm}
\hspace{-0.4cm}
\begin{minipage}{4.0cm}
\begin{lstlisting}[
  language=java,
  label=list:duplication-typecheck-opportunity-after,
  captionpos=t,
  numbers=left,
  numbersep=2pt
]
if (x instanceof C) {
  a(); c()
} else b()
\end{lstlisting}
\end{minipage}
\vspace{-0.5cm}
\end{wrapfigure}
After duplicating the second §instanceof§-check within both preceding branches,
this second check becomes dominated by the first check.
It can therefore be eliminated, resulting in the code shown on the left.

Since tail-duplication optimizations typically enable
other optimizations by devirtualizing the callsites,
we decided to include DBDS in the impact analysis.
We found that this optimization mostly affects ¡streams-mnemonics¡,
with a performance impact of around $22\%$.

% \wb{I think this writing style breaks the double-blind reviewing process.}
% \ap{Rephrased to say just that we thought tail-duplication might be important so we included it.}


==> sections/pca.tex <==
% !TEX root = ../main.tex

%Table~\ref{tab:complete-key-metrics} in Appendix~\ref{sec:app:metrics} 

%%%%%%%%%%%%%%%% THIS TABLE CONTAINS WARM-UPS
%%%%%%%%%%%%%%%% UNCOMMENT IT IF NEEDED

%\begin{table*}[t]
%\caption{Benchmarks considered in the paper, including input size, number of warm-up iterations (\# w.u.) and number of operations executed (\# ops). }
%\label{table:allworkloads}
%\centering \footnotesize
%\begin{tabular}{  l l | l l | l r l r  }
%\toprule
% {\bf Benchmark} & {\bf Input}  &  {\bf Benchmark} & {\bf Input}  & {\bf Benchmark} & \multirow{2}{*}{\bf \# ops} & \multirow{2}{*}{\bf Benchmark} & \multirow{2}{*}{\bf \# ops}\\
%{\bf DaCapo~\cite{Blackburn:2006:DBJ:1167515.1167488}} & {\bf size}   &  {\bf ScalaBench~\cite{Sewe:2011:DCC:2048066.2048118}} & {\bf size}   & {\bf SPECjvm2008~\cite{specjvm2008}}  & &  & \\
%\midrule
%\bench{avrora} & large  & \bench{actors} & huge  & \bench{compiler.compiler} & \num{20}  & \bench{scimark.lu.small} & \num{125}\\
%\hdashline[0.5pt/1pt]
%\bench{batik} & large  & \bench{apparat} & gargantuan  & \bench{compiler.sunflow}  & \num{20}& \bench{scimark.monte\_carlo} &\num{900}\\
%\hdashline[0.5pt/1pt]
%\bench{eclipse} & large  & \bench{factorie} & gargantuan  & \bench{compress} & \num{50} & \bench{scimark.sor.large} & \num{15}\\
%\hdashline[0.5pt/1pt]
%\bench{fop} & default & \bench{kiama} & default  & \bench{crypto.aes} & \num{20} & \bench{scimark.sor.small} & \num{75}\\
%\hdashline[0.5pt/1pt]
%\bench{h2} & huge  & \bench{scalac} & large  &\bench{crypto.rsa} & \num{150}  & \bench{scimark.sparse.large} & \num{10}\\
%\hdashline[0.5pt/1pt]
%\bench{jython} & large  & \bench{scaladoc} & large  & \bench{crypto.signverify} & \num{125} & \bench{scimark.sparse.small} & \num{25}\\
%\hdashline[0.5pt/1pt]
%\bench{luindex}  & default  & \bench{scalap} & large  & \bench{derby} & \num{30} & \bench{serial} & \num{25}\\
%\hdashline[0.5pt/1pt]
%\bench{lusearch-fix} & large  & \bench{scalariform} & huge  &\bench{mpegaudio} & \num{50} & \bench{sunflow} & \num{30}\\
%\hdashline[0.5pt/1pt]
%\bench{pmd} & large  & \bench{scalatest} & default  & \bench{scimark.fft.large}  & \num{10} & \bench{xml.transform} & \num{7}\\
%\hdashline[0.5pt/1pt]
%\bench{sunflow} & large  & \bench{scalaxb} & huge  & \bench{scimark.fft.small} & \num{100} & \bench{xml.validation} & \num{40}\\
%\hdashline[0.5pt/1pt]
%\bench{tomcat} & huge  & \bench{specs} & large  & \bench{scimark.lu.large} & \num{4} \\
%\hdashline[0.5pt/1pt]
%\bench{tradebeans} & huge  & \bench{tmt} & huge  &\\ 
%\hdashline[0.5pt/1pt]
%\bench{tradesoap} &  huge  &&&&&&\\
%\hdashline[0.5pt/1pt]
%\bench{xalan} & large   &&&&&&\\
%\bottomrule
%\end{tabular} 
%\end{table*}






%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%


Having collected the metrics described in Section \ref{sec:metric-comparison},
we used these metrics to narrow down the list of benchmarks,
and to compare Renaissance to the established benchmark suites.
In this section, we show that Renaissance represents the selected concurrency primitives
better than the existing suites,
that it is comparable to suites such as DaCapo and ScalaBench
in terms of object-allocation rates and dynamic dispatch,
and that it exercises §invokedynamic§ more often.


\subsection{Benchmark Suites}

We compare Renaissance with benchmarks included in several established 
and widely-used benchmark suites for the JVM:
DaCapo~\cite{Blackburn:2006:DBJ:1167515.1167488}, 
ScalaBench~\cite{Sewe:2011:DCC:2048066.2048118},
and SPECjvm2008~\cite{specjvm2008}.\footnote{
  We use the latest released versions of the suites at the time of writing:
  \mbox{DaCapo v.9.12-MR1} (dated Jan.~2018),
  \mbox{ScalaBench} v.0.1.0 (dated Feb.~2012)
  and \mbox{SPECjvm2008 v.1.01} (dated May~2009).
  According to the guidelines on the DaCapo website,
  we use the \bench{lusearch-fix} benchmark instead of \bench{lusearch}.
} 
%\footnote{Results reported on \bench{lusearch} have been obtained on \bench{lusearch-fix}.}
These suites can be executed with different input sizes.
In DaCapo and ScalaBench, 
we use the largest input defined for each benchmark, while in SPECjvm2008 
we use the ``lagom'' workload
(a fixed-size workload executing a given number of operations,
intended for research purposes~\cite{spec-manual}).
Table~\ref{table:allworkloads} in Section~\ref{sec:app:benchmarks}
of the supplemental material lists all benchmarks that we considered. 
%along with the used input sized, expressed as number of operations executed in SPECjvm2008.
%\ap{
%Space-wise, I think we should put these tables into the appendix.
%They add quite detailed information to the paper, and they take a lot of space.
%}

%\ar{This paragraph might be tuned (or separated in its own section)
%according to the experimental setup described in following sections.}
All benchmarks have a \emph{warm-up} phase, 
which takes either a number of iterations (Renaissance, DaCapo, ScalaBench) 
or some execution time (SPECjvm\-2008).
Execution after the warmup is classified as \emph{steady-state},
and we always measure steady-state execution in this paper.


%We let benchmarks warm up until dynamic compilation 
%and GC ergonomics are stabilized, following the methodology 
%of Lengauer et al.~\cite{Lengauer:2017:CJB:3030207.3030211}. 
%Table~\ref{table:allworkloads} lists the benchmarks considered. For DaCapo and ScalaBench, 
%the table shows the used input size and the number of warm-up iterations
%(in the last column). For SPECjvm2008, we report  the number of operations
%executed with the ``lagom'' workload on our machine. 
%Warm-up time for all SPEC benchmarks is set to 20 seconds. 
%The number of warm-up iterations for Renaissance are shown 
%in Table~\ref{tab:benchmarks}. \ar{Check later the addition of warm-ups to table 1.}





\subsection{Methodology}

To study the differences between Renaissance and other suites, we first collect the metrics
defined in Section~\ref{sec:metric-comparison} for all workloads;%
\footnote{
\forcameraready{
Table~\ref{tab:pcametricsext} in Section~\ref{sec:app:metrics}
of the supplemental material reports
the collected unnormalized metrics for all analyzed benchmarks.
}
} 
then, we visually 
compare them by means of scatter plots. Rather than analyzing benchmarks on a 
coordinate system composed of 11~dimensions (one dimension for each collected metric)
we resort to \emph{principal component analysis (PCA)}~\cite{doi:10.1080/14786440109462720}
to reduce data dimensionality, comparing benchmarks on the resulting coordinate system. 
PCA is a statistical technique that transforms
a $K$-dimensional space into another space of linearly uncorrelated variables,
called \emph{principal components} (PCs). PCA applies linear transformations such that the
first PC has the largest possible variance, while each subsequent 
component has the highest possible variance, under the constraint of being orthogonal 
to the preceeding components. Considering variance as a measure of information, 
PCA allows one to reduce the dimensionality of the original dataset by considering only 
the first components (i.e., those retaining most of the variance) while preserving 
as much information as possible from the original dataset. 

We apply PCA as follows. Matrix $\mathbf{X}$ contains the set of collected metrics. 
Each component $x_{ij} \in X$ ($i \in [1,N]$; $j \in [1, K]$;
where $N$ is the number of benchmarks  analyzed and $K$ the number of collected metrics)
is the normalized value of metric~$j$ obtained on benchmark~$i$.
The metrics are profiled during a single steady-state benchmark execution, 
as discussed in more details in Section~\ref{sec:app:pca:settings}
of the supplemental material.
%Before collecting the metrics, we let the benchmarks warm-up until dynamic compilation
%and GC ergonomics are stabilized, following the methodology 
%of Lengauer et al.~\cite{Lengauer:2017:CJB:3030207.3030211}. 

%Table~\ref{table:allworkloads} lists the benchmarks considered. For DaCapo and ScalaBench, 
%the table shows the used input size and the number of warm-up iterations
%(in the last column). For SPECjvm2008, we report  the number of operations
%executed with the ``lagom'' workload on our machine. 
%Warm-up time for all SPEC benchmarks is set to 20 seconds. 
%The number of warm-up iterations for Renaissance are shown 
%in Table~\ref{tab:benchmarks}. \ar{Check later the addition of warm-ups to table 1.}
 
 
Each metric vector $X_j$ is standardized to zero mean and unit variance, yielding a new vector 
$Y_j = \frac{X_j - \overline{x_j}}{s_j} \in \mathbf{Y}$ (where $\overline{x_j}$ and
 $s_j$ are the mean and variance of $X_j$, respectively). 
 According to established practices, we apply PCA
on the standardized matrix $\mathbf{Y}$ rather than on $\mathbf{X}$.
% to reduce the difference between data with different domains. \ar{Double-check}. 
PCA produces a new matrix 
%$\mathbf{Z} = \{Z_i\}$  %where $Z_i = \sum_{j = 1}^{N}a_{ij}Y_i ~(a_{ij} \in [-1, 1])$. 
%where 
%$Z_i$ is the $i$-th principal component (henceforth called PC$i$), 
%while each $z_{ij} \in Z_i$ ($j  \in [1,K]$) express the contribution of metric $j$ to PC$i$. 
$\mathbf{S} = \mathbf{Y}\mathbf{L}$, where each row vector in $\mathbf{S}$ 
 is the projection of the corresponding row vector in $\mathbf{Y}$ on 
the new coordinate system formed by the PCs (called \emph{score}), while $l_{ij} \in \mathbf{L}$
($l_{ij} \in [-1,1]; i, j \in [1,K]$)
is the \emph{loading} of metric $i$ on the $j$-th PC (henceforth called PC$j$). 
The absolute value of a loading quantifies the correlation of a metric to a given PC,
while its sign determines if the correlation is positive or negative.




\subsection{Analysis}

\begin{table}[t]
\caption{Loadings of metrics (defined in Table~\ref{tab:metrics}) on the first four principal components (PCs), sorted by absolute value (descending order).} %\ar{As an alternative, this table can be merged with Table 2, reporting only the rank and the sign of the loadings, as in the DaCapo paper. }}
\label{table:pca:loadings}
\centering \scriptsize
\begin{tabular}{ p{8mm}r | p{8mm}r | p{8mm}r | p{8mm}r}
\hline
\multicolumn{2}{c|}{\bf PC1} & \multicolumn{2}{c|}{\bf PC2} & \multicolumn{2}{c|}{\bf PC3} & \multicolumn{2}{c}{\bf PC4}\\
 {\bf Metric} &  {\bf load.} & { \bf Metric} &  { \bf load.}   & {\bf Metric} &  {\bf load.} & { \bf Metric} &  { \bf load.}\\ 
\hline
\metric{object} & {\tt +0.50} & \metric{atomic} & {\tt +0.67} & \metric{cachemiss} & {\tt +0.58} & \metric{idynamic} & {\tt +0.56}\\\hdashline[0.5pt/1pt]
\metric{cpu} & {\tt -0.49} & \metric{park} & {\tt +0.65} & \metric{notify} & {\tt +0.50} &\metric{array} & {\tt +0.42}\\\hdashline[0.5pt/1pt]
\metric{method} & {\tt +0.44} & \metric{method} & {\tt +0.20} &\metric{wait} & {\tt +0.41} & \metric{notify} & {\tt +0.42}\\\hdashline[0.5pt/1pt]
\metric{array} & {\tt +0.40} & \metric{notify} & {\tt +0.18} & \metric{cpu} & {\tt -0.28} & \metric{method} & {\tt -0.35}\\\hdashline[0.5pt/1pt]
\metric{idynamic} & {\tt +0.27} & \metric{idynamic} & {\tt -0.17} & \metric{synch} & {\tt -0.25} & \metric{cachemiss} & {\tt +0.28}\\\hdashline[0.5pt/1pt]
\metric{synch} & {\tt -0.17} & \metric{cpu} & {\tt -0.16} & \metric{park} & {\tt -0.20} & \metric{cpu} & {\tt +0.22}\\\hdashline[0.5pt/1pt]
\metric{notify} & {\tt -0.13} & \metric{cachemiss} & {\tt -0.08} & \metric{idynamic} & {\tt -0.18} & \metric{atomic} & {\tt +0.18}\\\hdashline[0.5pt/1pt]
\metric{atomic} & {\tt -0.13} & \metric{object} & {\tt +0.05} & \metric{array} & -{\tt 0.13} & \metric{wait} &{\tt  -0.15}\\\hdashline[0.5pt/1pt]
\metric{cachemiss} & {\tt -0.07} & \metric{array} & {\tt -0.03} & \metric{method} & {\tt +0.10} & \metric{object} & {\tt +0.13}\\\hdashline[0.5pt/1pt]
\metric{park} & {\tt -0.06} & \metric{synch} & {\tt -0.02} & \metric{object} & {\tt -0.04} & \metric{synch} & {\tt +0.11}\\\hdashline[0.5pt/1pt]
\metric{wait} & {\tt -0.02} & \metric{wait} & {\tt -0.00} & \metric{atomic} & {\tt -0.03} & \metric{park} & {\tt +0.05}\\
\hline
\end{tabular} 
\end{table}

\begin{figure}[t]
\subfigure[PC1 vs PC2.]{
\label{subfig:pca:1vs2}
\includegraphics[width=0.46\columnwidth]{figures/pca1}
}
\subfigure[PC3 vs PC4.]{
\label{subfig:pca:3vs4}
\includegraphics[width=0.46\columnwidth]{figures/pca2}
}
\caption{Scatter plots of benchmark scores over the first four principal components (PCs).}
\label{fig:pca:scatter}
\end{figure}

Table~\ref{table:pca:loadings} reports the loading of each metric
on the first four PCs, ranked %is performed by sorting the loadings for a given PC
by their absolute values %\wb{Please double check whether the rephrased sentence is accurate.} 
in descending order,
%(e.g., \metric{object} has rank of 1 for PC1, 
%because the loading of \metric{object} has the highest absolute value among 
%all metrics for PC1). The sign  before each rank denotes whether the correlation
%is positive (+) or negative (-). 
while in Figure~\ref{fig:pca:scatter}, we plot the scores 
of the considered benchmarks against the four PCs.
\footnote{
A larger version of Figure~\ref{fig:pca:scatter} can be found
in Section~\ref{sec:app:pca:larger} of the supplemental material.
}
The first four components account for $\sim$60\% of the variance present in the data.
\footnote{
As discussed in Section~\ref{sec:app:pca:settings} of the supplemental material,
we excluded benchmarks \bench{tradebeans}, \bench{actors} and
\bench{scimark.monte\_carlo} from the PCA.
}
%  due to the excessive amount of time needed to profile  this benchmark, exceeding 7~days.
%}.


% the loadings of the key metrics on 
%the first four principal components (which account for the 60\% of the variance 
%present in the data), while Figure~\ref{fig:pca:scatter} plots the considered 
%benchmarks against the four principal components.\footnote{In this footnote, 
%list benchmarks that couldn't be put in PCA because of failures in profiling}
%
As shown in Table~\ref{table:pca:loadings},
object allocation, dynamic dispatch, and array allocation correlate positively with PC1,
% abstractions of object-oriented programming 
% (i.e., \metric{object} and \metric{method})
and CPU utilization correlates negatively.
Figure~\ref{subfig:pca:1vs2} shows that 
the SPECjvm2008 benchmarks are clustered in the bottom-left portion of the figure, 
while the benchmarks of the other suites are well distributed along PC1.
This is a sign that Renaissance, DaCapo and ScalaBench
contain applications that nicely exercise object allocation and dynamic dispatch,
which is often a sign of using abstractions in those workloads.
% Moreover, Renaissance includes one benchmark (\bench{streams-mnemonics})
% that particularly makes use of such features,
% to a significantly higher degree than the other analyzed benchmarks.
% \ap{This might some wild lambda object allocation inside a nested stream operation too}


In contrast, PC2 exhibits a strong positive correlation with two concurrency primitives,
i.e., \metric{atomic} and \metric{park}.
As demonstrated by the wide distribution of Renaissance benchmarks
along PC2, as shown in Figure~\ref{subfig:pca:1vs2},
Renaissance benchmarks extensively use these primitives.
On the other hand, benchmarks from the other suites span a limited space along PC2.
Similarly to PC2, PC3 is well correlated with metrics estimating concurrency,
particularly cache misses and the usage of §wait§/§notify§.
The benchmark distribution %\wb{What is a benchmark trend?} 
along PC3 is similar to the one along PC2
(as shown in Figure~\ref{subfig:pca:3vs4}), which suggests that generally,
the use of concurrency primitives in DaCapo, ScalaBench, and SPECjvm2008 is limited. 
%The outliers in these suites along PC3 are caused by an 
%exceptionally high cache-miss rate (i.e., \bench{avrora} and \bench{tmt}) and 
%wait/notify usage (\bench{derby}).
%observed in such benchmarks.  %\ar{Show the 3 outliers in the plot for other benchmark suite as well}.

%\ap{
%1. The cache miss rate seems weird.
%2. I thought that avrora is due to wait/notify
%3. I think it's important to only claim things we are 100\% sure about.
%It might make sense to remove those claims about PC3.
%Less is more.
%}

Finally, \metric{idynamic} contributes most to PC4, with a strong positive correlation.
The presence of numerous Renaissance benchmarks in the top part of Figure~\ref{subfig:pca:3vs4}
demonstrates the frequent execution of §invokedynamic§ bytecodes
in the workloads (indeed, 10 out of 21 benchmarks execute this bytecode at runtime), 
which in turn may represent the use of functional-style operations
commonly found in parallelism frameworks.
This is expected, as other suites were released before the introduction 
of §invokedynamic§ in JDK~7~\cite{jsr292} and of Lambas and Streams in JDK 8~\cite{jsr335}
(while a recent DaCapo version was released in Jan.~2018, 
there was no major change to the constituent benchmarks, originally released in~2009).
% The use of functional-style operations is also supported by the fact
% that array allocations have a strong
% correlation with this component, and arrays are frequently allocated by such operations. 

% \ap{Since we did not identify places in the code where Streams do array allocation,
% I would remove this last sentence.}

% Overall, the results demonstrate that Renaissance benchmarks use basic concurrency primitives 
% significantly more often than 
% %Renaissance has significantly more representative \wb{Representative for what?} 
% DaCapo, ScalaBench, and SPECjvm2008 workloads.
% %
% Moreover, several Renaissance benchmarks
% execute recent programming patterns which are 
% missing in other benchmark suites, and make use of complex code leveraging 
% the building blocks of 
% object-oriented programming. %\wb{You can't conclude this without analyzing the subtyping hierarchy and the use of abstractions for parameter and variable types.} 
% These features make Renaissance significantly diverse wrt. the other analyzed suites. %\wb{Diversity seems not the right word here.} 
% \ar{The validity of the following paragraph should be doublechecked when Sections 5/6 are ready}
%  In turn, such diversity can pinpoint
% performance improvements that are not possible to observe on DaCapo, ScalaBench, or SPECjvm2008. 
% One such example are JIT compiler optimizations \wb{For concurrency primitives?}, 
% discussed in the next section. 

% \ap{I would remove this paragraph, since it does not say anything new, fundamentally.}


==> sections/related.tex <==
% !TEX root = ../main.tex


By differentiating between the optimizations that are worth pursuing,
benchmark suites were at the core of innovation throughout the JVM's history.
Since its introduction in 2006,
the \mbox{DaCapo} suite~\cite{Blackburn:2006:DBJ:1167515.1167488}
has been a de facto standard for JVM benchmarking.
While much of the original motivation for the DaCapo suite
was to understand object and memory behavior in complex Java applications,
this suite is still actively used to evaluate not only JVM components
such as JIT compilers~\cite{Prokopec:2019:OII:3314872.3314893,Leopoldseder:2018:DDS:3179541.3168811,Prokopec:2017:MCO:3136000.3136002,Eisl:2016:TRA:2972206.2972211,Stadler:2014:PEA:2581122.2544157}
and garbage collectors~\cite{Akram:2018:WGC:3192366.3192392,Nguyen:2016:YHB:3026877.3026905},
but also tools such as profilers~\cite{Schorgenhumer:2017:ESL:3030207.3030234,Bruno:2017:PAP:3135974.3135986},
data-race detectors~\cite{Biswas:2017:LDR:3033019.3033020,Wood:2017:IBD:3152284.3133893},
memory monitors and contention analyzers~\cite{Weninger:2018:UCM:3184407.3184412,Hofer:2016:ETV:2851553.2851559},
static analyzers~\cite{Grech:2018:SHU:3213846.3213860,Thiessen:2017:CTP:3062341.3062359},
and debuggers~\cite{Liu:2018:DFC:3192366.3192390}.

The subsequently proposed
\mbox{ScalaBench} suite~\cite{Sewe:2011:DCC:2048066.2048118,Sewe:2012}
identified a range of typical Scala programs,
and argued that Scala and Java programs have considerably different
distributions of instructions,
polymorphic calls, object allocations, and method sizes.
This observation that benchmark suites tend to over-represent
certain programming styles was also noticed in other languages,
(e.g., JavaScript~\cite{Ratanaworabhan:2010:JCB:1863166.1863169}).
%
On the other hand,
the \mbox{SPECjvm2008} benchmark suite~\cite{specjvm2008}
focused more on the core Java functionality.
Most of the \mbox{SPECjvm2008} benchmarks are considerably smaller
than the \mbox{DaCapo} and \mbox{ScalaBench} benchmarks,
and do not use a lot of object-oriented abstractions --
\mbox{SPECjvm2008} exercises classic JIT compiler optimizations,
such as instruction scheduling and loop optimizations~\cite{duboscq-thesis}.

\forcameraready{We did not include SPECjbb2015~\cite{specjbb2015} in our analysis,
because it consists of a single benchmark designed to run over
2~hours, typically executed on multiple JVM instances. Using
SPECjbb2015 to detect small statistically significant changes
is therefore relatively costly (needs long execution time).
A brief evaluation suggests that the combined effect of all
optimizations considered here accounts for about 1.2\%
improvement in the reported peak throughput (max jOPS)
in single JVM configuration.}

Another older JVM benchmark suite is Java Grande~\cite{1592782},
but it consists mostly of microbenchmarks.

% \wb{I'm not sure this is a good justification for excluding SPECjbb2015. We're
% interested in a broad range of modern, concurrent workloads, and whether we observe
% a difference between C2 and Graal should not be stated as a benchmark selection criterion.}
% \ap{Commented that we did not notice anything interesting.}

The tuning of compilers such as C2~\cite{Paleczny:2001:JHT:1267847.1267848}
and Graal~\cite{graalvm-download,Duboscq:2013:IRS:2542142.2542143}
was heavily influenced by the \mbox{DaCapo}, \mbox{ScalaBench}, and \mbox{SPECjvm2008} suites.
Given that these existing benchmark suites do not exercise
many frameworks and language extensions that gained popularity in the recent years,
we looked for workloads exercising frameworks such as
Java Streams~\cite{jep107} and Parallel Collections~\cite{prokopec11,7092728,Prokopec:196627},
Reactive Extensions~\cite{rx},
Akka~\cite{akka},
Scala actors~\cite{Haller:2007:AUT:1764606.1764620}
and Reactors~\cite{Prokopec:2015:ICE:2814228.2814245,Prokopec:2016:PSR:3001886.3001891,Prokopec:2017:EBB:3133850.3133865,Prokopec:2014:CAM:2637647.2637656},
coroutines~\cite{kotlin-coroutines,DBLP:conf/ecoop/ProkopecL18,coroutines-tech-report},
Apache~Spark~\cite{Zaharia:2010:SCC:1863103.1863113},
futures and promises~\cite{SIP14},
Netty~\cite{github-netty},
Twitter~Finagle~\cite{github-finagle},
and Neo4J~\cite{github-neo4j}.
Most of these frameworks either assist in structuring concurrent programs,
or enable programmers to declaratively specify data-parallel processing tasks.
In both cases, they achieve these goals by providing a higher level of abstraction --
for example, Finagle supports functional-style composition of future values,
while Apache~Spark exposes data-processing combinators for distributed datasets.
By inspecting the IR of the open-source Graal compiler
(c.f. Section~\ref{sec:compiler-optimizations}),
we found that many of the benchmarks
exercise the interaction between different types of JIT compiler optimizations:
optimizations, such as inlining, duplication~\cite{Leopoldseder:2018:DDS:3179541.3168811},
and partial escape analysis~\cite{Stadler:2014:PEA:2581122.2544157},
typically start by reducing the level of abstraction in these frameworks,
and then trigger more low-level optimizations such as
guard motion~\cite{duboscq-thesis}, vectorization, or atomic-operation coalescing.
Aside from a challenge in dealing with high-level abstractions,
the new concurrency primitives in modern benchmarks pose new optimization opportunities,
such as contention elimination~\cite{Lu:2001:CER:379539.379568},
application-specific work-stealing~\cite{10.1007/978-3-319-09967-54},
NUMA-aware node replication~\cite{Calciu:2017:BCD:3037697.3037721},
speculative spinning~\cite{Prokopec2017},
access path caching~\cite{Prokopec:2018:CCL:3178487.3178498,Prokopec2018,techreport-17-prokopec,cache-trie-remove-dataset},
or other traditional compiler optimizations applied to concurrent programs~\cite{Sevcik:2011:SOS:1993498.1993534}.
Many of these newer optimizations may be applicable to domains
such as concurrent data structures, which have been extensively studied
on the JVM~\cite{Oshman:2013:SLC:2484239.2484270,Prokopec2016,cliffclick,prokopec12ctries,EPFL-REPORT-166908,Prokopec2011,Basin:2017:KKM:3018743.3018761,Prokopec:2015:SLQ:2774975.2774976,bronsonavl,prokopec12flowpools,dougleahome}.

Unlike some other suites whose goal
was to simulate deployment in clusters and Cloud environments,
such as CloudSuite~\cite{Ferdman:2012:CCS:2248487.2150982},
our design decision was to follow the philosophy of \mbox{DaCapo} and \mbox{ScalaBench},
in which benchmarks are executed within a single JVM instance,
whose execution characteristics can be understood more easily.
Still, we found some alternative suites useful:
for example, we took the ¡movie-lens¡ benchmark for Apache~Spark from CloudSuite,
and we adapted it to use Spark's single-process mode.

The Unbalanced Cobwebbed Tree (UCT) benchmark~\cite{Zhao:2013:LBN:2541329.2541337}
was designed for better actor-scheduler comparison on non-uniform workloads,
and our ¡akka-uct¡ benchmark is the implementation of that benchmark
in the Akka actor framework for the JVM~\cite{akka}.
A suite that specialized exclusively on benchmarks for the actor model
is the Savina suite~\cite{Imam:2014:SAB:2687357.2687368}.

Several other benchmarks were either inspired by or adapted from existing workloads.
The ¡naive-bayes¡, ¡log-regression¡, ¡als¡, ¡dec-tree¡ and ¡chi-square¡ benchmarks
directly work with several machine-learning algorithms from Apache~Spark MLLib,
and some of these benchmarks were inspired by the \mbox{SparkPerf} suite~\cite{spark-perf}.
The \emph{Shakespeare plays Scrabble} benchmark~\cite{scrabble-benchmark}
was presented by José Paumard at the Virtual Technology Summit~2015
to demonstrate an advanced usage of Java Streams,
and we directly adopted it as our ¡scrabble¡ benchmark.
The ¡rx-scrabble¡ is a version of the ¡scrabble¡ benchmark
that uses the Reactive Extensions framework instead of Java Streams.
The ¡streams-mnemonics¡ benchmark is rewritten
from the \emph{Phone Mnemonics} benchmark that was originally used
to demonstrate the usage of Scala collections~\cite{state-of-scala}.
The ¡stm-bench7¡ benchmark is STMBench7~\cite{Guerraoui:2007:SBS:1272996.1273029}
applied to ScalaSTM~\cite{scala-stm-expert-group,Bronson10ccstm:a},
a software transactional memory implementation for Scala,
while the ¡philosophers¡ benchmark is
ScalaSTM's \emph{Reality-Show Philosophers} usage example.

% \wb{I think we should also mention the Java Grande benchmarks, as they include multi-threaded
% benchmarks (representing numerically intensive applications). It seems they have been ported to
% JMH.}\ar{An argument against Java Grande (but not against citing it) is that they are old. Some
% of their workloads don't even use thread pool...}
% \ap{mentioned above}


